Strong Gaussian Approximation for the Sum of Random Vectors

This paper derives a new strong Gaussian approximation bound for the sum of independent random vectors. The approach relies on the optimal transport theory and yields \textit{explicit} dependence on the dimension size $p$ and the sample size $n$. This dependence establishes a new fundamental limit for all practical applications of statistical learning theory. Particularly, based on this bound, we prove approximation in distribution for the maximum norm in a high-dimensional setting ($p >n$).

==> bernulli2020(4)/bridge.tex <==
\noindent Here we will use a specified for the Wasserstein distance version of Stein's method \cite{stein_meth} proposed in paper \cite{Bonis}. For that define a smooth transition from  $\xiv$ to $\gammav$ parametrized by $t$:
\begin{equation} \label{tranz_def}
X_t = e^{-t} \xiv + \sqrt{1 - e^{-2t}} \gammav, \quad t \in [0, \infty].
\end{equation}
\begin{remark}
The choice of this particular transition is explained by the fact that Markov process $X_t$ has generator $A f(x) = \nabla^T \Sigma \nabla f(x) - x^T \nabla f(x)$ and Gaussian stationary measure \cite{bakry_hal}. It is also known as Ornstein--Uhlenbeck process.  
\end{remark}

\noindent Further we will require one important property of this process that will help us to find an upper bound for the derivative of $W_L$ by $t$. It was proposed in paper \cite{OttoVillani} that deals with particular case derivative estimation of $W_2$. There exists a function $\mathcal{G}_t(x)$ that effects the transition of  measure $\mu_t(x)$ of $X_t$ in the following way $\forall f \in \mathbb{C}^1$:
\begin{equation} \label{phi_def}
\frac{d}{dt} \int f(x) d \mu_t(x)  =  \int \nabla^T f(x) \nabla \mathcal{G}_t(x) d \mu_t(x),
\quad t \in [0, \infty).
\end{equation}


\noindent  Its gradient has explicit representation 
\[
\nabla \mathcal{G}_t(X_t) = \E \left[ \frac{d}{dt} X_t \bigg | X_t \right],
\]
since 
\[
\lim_{\Delta \to 0} \frac{\E f(X_{t + \Delta}) - \E f(X_{t}) }{\Delta} = \lim_{\Delta \to 0} \E \nabla^T f(X_t) \frac{\E [ X_{t + \Delta} - X_{t} | X_t ] }{\Delta} = \E \nabla^T f(X_t) \E \left[ \frac{d}{dt} X_t \bigg | X_t \right].  
\]
And differentiating equation (\ref{tranz_def}) by time we derive that 

\begin{equation}\label{phi_expl_def}
\nabla \mathcal{G}_t(X_t) = - e^{-t} \E \left( X_0 - \frac{e^{-t}}{\sqrt{1 - e^{-2t}}} X_\infty \bigg| X_t \right).
\end{equation}

\noindent The next result allows us to bound an 
increment the of Wasserstein distance in a small interval of the transition parameter $t$. 

\begin{lemma} \label{was_int_bound} Let $\nabla \mathcal{G}_t(X_t) \in \R^p$, $t \in [0, \infty] $ be uniformly continuous and bounded random process.  For any cost function $c(x-y)$ in Wasserstein distance $W(c)$ and infinitely small time shift $ds$ it holds
\[
W(c)(X_{t}, X_{t + ds})  \leq \E c \big(ds \nabla \mathcal{G}_t  (X_{t})\big)
\]
and moreover if $\exists f: \R \to \R$ such that  $\forall t,s \geq 0$
\begin{equation}\label{Wtriangle}
f\left \{ W(c)(X_0, X_{t+s}) \right\} -  f\left\{W(c)(X_0, X_{t}) \right\} \leq f \{W(c)(X_t, X_{t+s}) \}  
\end{equation}
then for any $a, b \geq 0$
\[
f\{W(c)(X_a, X_b)\} \leq
\int_{a}^{b} \frac{f \left\{ \E c(ds \nabla \mathcal{G}_t)  
\right \}}{ds} dt .
\]
Particularly, if $c(x-y)$ is any norm in power $L$, then 
\[
W_L(X_a, X_b) \leq
\int_{a}^{b}  \left\{ \E \| \nabla \mathcal{G}_t \|^L  
\right \}^{1/L} dt .
\]
\end{lemma}

\begin{proof} Fix an arbitrary point $t$. Define a new mapping $T_{s}$ on the space of the random variable $X_t$ by equation 
\begin{equation}\label{Tdef}
\frac{\partial}{\partial s} T_{s}(x) =   \nabla \mathcal{G}_{t+s} (T_{s}(x)), 
\quad  T_0(x) = x, \quad s \geq 0.
\end{equation}
It turns out that function $x \to T_{s}(x)$ is the push-forward transport mapping, such that $X_{t+s} =  T_{s}(X_t)$ in distribution (see proof of Lemma 2 in \cite{OttoVillani}). In order to be consistent with our notation we provide below another proof of this proposition.  
Note that for an arbitrary functions $h \in C^1$ and $h_s = h(T^{-1}_s)$ it holds 
\[
\frac{d}{ds}h_s(T_s) = \frac{\partial}{\partial s}h_s(T_s) + \nabla^T h_s(T_s)  \frac{\partial}{\partial s} T_{s}  = 0
\]and with differential equation for $T_s$  (\ref{Tdef})  one gets 
\[
\forall x \in \Omega(X_t) : \quad
\frac{\partial}{\partial s}h_s(x) = -  \nabla^T \mathcal{G}_{t+s}(x) \nabla h_s(x).
\]Then involving  property (\ref{phi_def})  leads to 
\[
\frac{d}{ds} \int h_s(x) d \mu_{t+s}(x) 
=  \int \frac{\partial}{\partial s} h_s(x)  + \nabla^T \mathcal{G}_{t+s}(x) \nabla h_s(x) d \mu_{t+s}   = 0.
\]It proves that $T_s^{-1}(X_{t+s}) = X_t$ and subsequently $X_{t+s} = T_s T_s^{-1}(X_{t+s}) = T_s(X_t)$. 
By the definition of Wasserstein distance and the push-forward transport mapping $T_s$  (\ref{Tdef})
\[
W(c)(X_{t}, X_{t + ds}) \leq \E c \big(T_{ds}(X_t) - T_{0}(X_t) \big) = \E c \big(ds \nabla \mathcal{G}_t  (X_{t})\big)
\]and consequently with the triangle inequality assumption (\ref{Wtriangle})  
\[
\frac{d}{dt} f\{ W(c) (X_0, X_t) \} \leq  \frac{1}{ds}f \{ W(c)(X_{t}, X_{t + ds})\} 
\leq \frac{1}{ds}f \{ \E c (ds \nabla \mathcal{G}_t  (X_{t})) \}.
\]
After the integration we obtain the second statement of this lemma. In case $c(x-y) = \| x-y \|^L$ we set $f = \sqrt[L]{}$ and apply equality 
\[
  \E \| ds \nabla \mathcal{G}_t  (X_{t}) \|^L  =  (ds)^L \E  \| \nabla \mathcal{G}_t  (X_{t}) \|^L .
\]
\end{proof}

\noindent Involve a sequence of useful lemmas that will help us to estimate term $\E  \| \nabla \mathcal{G}_t  (X_{t}) \|^L $ from the previous result.

\begin{lemma} [Rosenthal's inequality \cite{rosental}] \label{rose} For all martingales $S_k = \sum_{i=1}^k{\zetav_i}$ and $2 \leq q < \infty$:
\[
\left [ \E \max_{0 \leq k < \infty} \| S_k \|^q  \right]^{1/q} \leq \frac{C q}{\log q} \left[  \E \left(   \sum_{i=1}^\infty \E_{i-1} \| \zetav_i \|^2  \right)^{q/2} + \E \max_{0 \leq i < \infty} \| \zetav_i \|^q \right]^{1/q}.
\]   
By $\E_{i-1}$ we denote conditional expectation on previous values of the martingale $S_0, \ldots,S_{i-1}$ and by definition $\zetav_i$ are increments of the martingale which may be dependent in general case. 
\end{lemma}

\begin{lemma} \label{boni} \cite{Bonis} Let $\gammav \in \ND(0, I)$ and for all $\alpha \in \N^p$: $x_\alpha \in \R^p$ and $H_\alpha(\gammav, \Sigma)$ be the multivariate Hermite polynomials, defined by 
\begin{equation}\label{Hdef2}
H_{\alpha}(\gammav, \Sigma) = (-1)^{| \alpha |} e^{\frac{ \gammav^T \Sigma^{-1} \gammav } {2}} \partial^{\alpha} e^{-\frac{  \gammav^T \Sigma^{-1} \gammav } {2}},
\quad
H_{\alpha}(\gammav) = H_{\alpha}(\gammav, I).
\end{equation}
 Then
\[
\left [ \E \normX{ \sum_\alpha x_\alpha H_\alpha(\gamma)  }^q \right]^{2/q} \leq \sum_\alpha \max (1, q-1)^{|\alpha|} \alpha! \normX{x_\alpha }^2.
\]
\end{lemma}

\begin{corollary} \label{boni_cons} In general case one may use coordinates replacement and property $\nabla_{(Ax)} = A^{-1} \nabla_x$, such that
\[
\left [ \E \normX{ \sum_{\alpha \geq 0} x_\alpha H_\alpha(\gamma, \Sigma)  }^q \right]^{2/q} \leq \sum_{\alpha \geq 0}  \max (1, q-1)^{|\alpha|} \alpha! \normX{ (\Sigma^{-1/2} x)_\alpha }^2.
\]
\end{corollary}

\noindent Combine the previous two lemmas. 

\begin{lemma} \label{Hsum}  Let $\gammav \in \ND(0, \Sigma)$ and for all $\alpha \in \N^p$: $\zetav^\alpha  \in \mathcal{P}(\R^p)$ and $H_\alpha(\gammav, \Sigma)$ be the multivariate Hermite polynomials (\ref{Hdef2}) and $\zetav^\alpha = \sum_i \zetav_i^\alpha$, where $\{ \zetav_i^\alpha\}$ are independent random vectors. Then for~$2 \leq q < \infty$
\begin{align*}
&\left [ \E \normX{ \sum_{i, \alpha}  \zetav_i^\alpha H_\alpha(\gamma, \Sigma)  }^q \right]^{1/q} \\
&\leq  C(q) \left[  \sum_{i, \alpha}  \alpha! (q-1)^{|\alpha|} \E \normX{\Sigma^{-1/2} \zetav_i^\alpha}^2   \right]^{1/2} \\
& +  \left[  \sum_{\alpha}  \alpha! (q-1)^{|\alpha|}  \normX{\Sigma^{-1/2} \E \zetav^\alpha}^2   \right]^{1/2} \\
&+ C(q) \left[ \sum_i \E \left( \sum_{\alpha}  \alpha! (q-1)^{|\alpha|} \normX{\Sigma^{-1/2} \zetav_i^\alpha}^2  \right)^{q/2}  \right]^{1/q}.
\end{align*}
where one may take $C(q) = \frac{C q}{\log q}$ for some absolute constant $C$. 
\end{lemma}

\begin{proof}Without loss of generality assume $\Sigma = I$. Note that for a random variable $\xi$ operator $[\E \xi^q]^{1/q}$ is the probability norm $L_q$. Use notation 
\[
\delta = \left \| \normX{ \sum_{i, \alpha}  \zetav_i^\alpha H_\alpha(\gamma)  } \right \|_{L_q}.
\]
In order to construct a martingale one has to substitute expectation from each $X^{\alpha}$. 
 For that use the triangle inequality 
\[
\delta
\leq \left \| \normX{ \sum_{i, \alpha}  (\zetav_i^\alpha - \E[ \zetav_i^\alpha]) H_\alpha(\gamma)  } \right \|_{L_q}
+  \left \| \normX{ \sum_{i, \alpha}  \E [ \zetav_i^\alpha] H_\alpha(\gamma)  } \right \|_{L_q}.
\]
Without loss of generality assume that $\E[ \zetav_i^\alpha] = 0$, since $\| \zetav_i^\alpha - \E \zetav_i^\alpha \|_{L_q} \leq 2 \| \zetav_i^\alpha \|_{L_q}$.  Apply Lemma~\ref{boni}.
\[
\delta
\leq  \left\| \left(  \sum_{\alpha}  \alpha! (q-1)^{|\alpha|}  \normX{\sum_i \zetav_i^\alpha  }^2   \right)^{1/2}\right\|_{L_q} .
\]
Apply Lemma \ref{rose} for this hybrid norm and bound maximum by sum of components in power $q$.
\[  
\delta/ C(q) \leq  \left[  \sum_{i, \alpha}  \alpha! (q-1)^{|\alpha|} \E \normX{\zetav_i^\alpha}^2   \right]^{1/2} + \left[ \E \max_i \left(  \sum_{\alpha}  \alpha! (q-1)^{|\alpha|}  \normX{\zetav_i^\alpha}^2   \right)^{q/2} \right]^{1/q},
\]where
\[
   \max_i \left(  \sum_{\alpha}  \alpha! (q-1)^{|\alpha|}  \normX{\zetav_i^\alpha}^2   \right)^{q/2}  \leq 
   \sum_i  \left( \sum_{\alpha}  \alpha! (q-1)^{|\alpha|} \normX{\zetav_i^\alpha}^2  \right)^{q/2} . 
\]
\end{proof}

\begin{theorem} \label{WLT} Let $\gammav \in \ND(0,  \Sigma)$ and $\{\xiv_i\}_{i=1}^n$ be independent random vectors with zero mean and variance $\sum_i \E \xiv_i \xiv_i^T = \Sigma$  and with domain in $\R^p$. 
The Wasserstein distance between $\xiv =\sum_i \xiv_i$ and $\gammav$ with $\| x - y \|^L$ cost function, where $L \geq 2$, has the following upper bound 
\[
\frac{  W_L(\xiv, \gammav) }{\| \Sigma \|^{1/2}} \leq 
\frac{C \, L^{3/2} }{\log L } \left( \mu_4^{1/2} + \mu_{2L}^{1/L} \right) 
 + \frac{  \sqrt{2}  e^{1/2} L^{1/2} \mu_2 }{ \sqrt{n}} + \frac{ e^{1/2} L  \mu_3  }{2} \log(2n),
\]
where $C$ is some absolute constant and with $\xiv'_{i}$ independent copies of $\xiv_{i}$ 
\[
\mu_k =  \left\{ \sum_{i=1}^n \E \left \| \Sigma^{-1/2} (\xiv_{i} - \xiv'_{i}) \right \|^{k}\right\}.
\]
% Moreover, if all $\xi_{ik}$ are sub-Gaussian with exponential moment 
% \[
% \forall i,k: \,
% \log \E \exp \left \{  \frac{\lambda \xi_{ik}} {\sigma_{k}}  \right\} \leq \frac{\nu^2 \lambda^2 }{ 2n }
% \]
% Then with $L = \log (np)$ and $\nu \geq 1$
% \[
% W_{c}^{1/L}(\xiv, \gammav) \leq O\left( \frac{ \overline{\sigma}\, \nu^3  \log^{2} (np) }{\sqrt{n}} \right)
% \]
\end{theorem}

\begin{proof} 
% Denote by $\xiv'_{1}, \ldots, \xiv'_{n}$ independent copies  of $\xiv_{1}, \ldots, \xiv_{n}$.  
According to the base procedure of the Stein's method \cite{stein_meth} we should consequently replace random vectors $\xiv_i$  by their independent copies  $\xiv'_{i}$ trowing random index at each step. It allow to estimate change of some function of interest that depends on the transition process $X_t$ (\ref{tranz_def}) under condition that $\mu_t$ is stationary measure. In our case the function is $ \nabla \mathcal{G}_t(X_t)$ (\ref{phi_expl_def}). For a formal description   
involve two additional random vectors with random uniform index $I \in \{1,\ldots,n\}$
\[
\xiv'(t) = \xiv + (\xiv'_{I} - \xiv_{I}) \Ind_I(t),
\]
where
\[
\Ind_I(t) = \Ind \left[ \| \Sigma^{-1/2} ( \xiv'_{I}- \xiv_{I}) \| \leq \left( \frac{ e^{2t}-1 }{L} \right)^{1/2} \right],
\]
and
\[
\tauv(t)  = \E \left [ 
  \frac{n}{2} (\xiv' - \xiv) \left( 1 + \sum_{\alpha \geq 0} \frac{(\xiv' - \xiv)^\alpha H_{\alpha}(\gammav, \Sigma)}{\alpha! (e^{2t} - 1)^{|\alpha| / 2}} \right)
  \bigg | \xiv, \gammav
\right].
\]
We restrict term  $\|  \Sigma^{-1/2} (\xiv'_{I}- \xiv_{I}) \|$ from the upper side in order to prevent irregularity in random vector $\tauv(t)$ when $t \to 0$. Note that for any smooth function $f$ by construction of $\xiv'(t)$ (ref. Lemma 10 in \cite{Bonis})
\[
\E \tauv(t) f(X_t) = n \E  \left(X'_t - X_t \right) \frac{ f(X'_t) + f(X_t) }{2}  = 0,
\]
where $X'_t = e^{-t} \xiv'(t) + \sqrt{1 - e^{-2t}} \gammav$. And as a consequence $\E(\tauv (t)  | X_t) = 0$. So one may note that $\tauv(t)$ shifts process $X_t$ without changing the its measure. Oppositely $ \nabla \mathcal{G}_t(X_t) $ shifts $X_t$ outside its measure towards $\gammav$. On order to reduce the unconditional expectation of $ \nabla \mathcal{G}_t(X_t) $  we will substitute $\tauv(t)$ from it.        
Accounting to the definition of $\nabla \mathcal{G}_t(X_t)$ (\ref{phi_expl_def}) we obtain 
\[
 \nabla \mathcal{G}_t(X_t) =  \nabla \mathcal{G}_t(X_t) -  e^{-t} \E(\tauv (t)  | X_t) = -   e^{-t} \E \left( \xiv - \frac{ 1 }{\sqrt{e^{2t} - 1}} \gammav + \tauv(t) \bigg| X_t \right).
\]We have just added  zero component to the initial value of  $ \nabla \mathcal{G}_t(X_t) $. Below we will use Jensen's inequality moving the conditional expectation outside the norm and $\tauv(t)$  will decrease the expected value of the norm. Add notation $\Sigma_i = \E \xiv_i \xiv_i^T$ with evident property 
$
 \sum_{i=1}^n \Sigma_i = \Sigma.
$
Use a short notation $\E_{X_t}$ for the expectation operator with $X_t$ condition.  Unwrap the last expression with $ \nabla \mathcal{G}_t(X_t)$
\[
 \E \left( \xiv - \frac{ 1 }{\sqrt{e^{2t} - 1}} \gammav + \tauv(t) \bigg| X_t \right)
\]\begin{equation} 
\label{phi_plus_tau}
\begin{split}
& = \sum_{i=1}^n  \E_{X_t}  (\xiv_{i} - \xiv'_{i}) (1 - \Ind_i(t)) \\
 & + \frac{1}{\sqrt{e^{2t} - 1}} \E_{X_t}  \sum_{i=1}^n \left( \frac{(\xiv'_{i} - \xiv_{i}) (\xiv'_{i} - \xiv_{i})^T  \Ind_i(t)   }{2} - \Sigma_i \right) \Sigma^{-1} \gammav \\
 & + \sum_{\alpha \geq 2} \frac{1}{2 \alpha! (e^{2t} - 1)^{|\alpha|/2}} \E_{X_t} H_\alpha(\gammav, \Sigma) \sum_{i=1}^n  (\xiv'_{i} - \xiv_{i}) (\xiv'_{i} - \xiv_{i})^{\alpha}  \Ind_i(t).    
\end{split}
\end{equation}Use notations from Lemma \ref{Hsum} and set 
\[
\zetav_i^0 =   (\xiv_{i} - \xiv'_{i}) (1 - \Ind_i(t)).
\]For $|\alpha| = 1$
\[
\zetav_i^\alpha = \frac{1}{\sqrt{e^{2t} - 1}}  \left( \frac{(\xiv'_{i} - \xiv_{i}) (\xiv'_{i} - \xiv_{i})^\alpha  \Ind_i(t)   }{2} -   \frac{ \E (\xiv'_{i} - \xiv_{i}) (\xiv'_{i} - \xiv_{i})^\alpha    }{2}  \right).
\]
For $|\alpha| > 1$
\[
\zetav_i^{\alpha} =   \frac{1}{2 \alpha! (e^{2t} - 1)^{|\alpha| /2}}  (\xiv'_{i} - \xiv_{i})  (\xiv'_{i} - \xiv_{i})^{\alpha}  \Ind_i(t) .   
\]
Next we want no estimate the power $L$ of $ \sum_{i, \alpha}  \zetav_i^\alpha H_\alpha(\gamma, \Sigma)  $, $\alpha \in \N$. Define a normalized vector 
\[
\overline{\xiv}_i = \Sigma^{-1/2} (\xiv'_{i} - \xiv_{i}).
\] 
In the expressions below we are going to use the following inequalities $\forall \alpha > 0$
\[
\Ind_{i}(t) \leq \frac{1}{\| \overline{\xiv}_i  \|^{| \alpha |} }  \left(\frac{e^{2t} - 1}{L} \right)^{| \alpha | / 2},
\quad 1 - \Ind_{i}(t) \leq \| \overline{\xiv}_i  \|^{| \alpha | } \left(\frac{L}{e^{2t} - 1} \right)^{ | \alpha | / 2}.
\]Note that $\forall l > 0$
\[
\| \zetav_i^0 \| \leq  \| \xiv'_{i} - \xiv_{i} \| \| \overline{\xiv}_i  \|^{l} \left(\frac{L}{e^{2t} - 1} \right)^{l/2},
\]
\[
\sum_{|\alpha| = 1 } \|\zetav_i^\alpha \|^2 \leq  \frac{ \| \xiv'_{i} - \xiv_{i} \|^2 \| \overline{\xiv}_i  \|^2     }{4 (e^{2t} - 1)}  +  \frac{  (\E \| \xiv'_{i} - \xiv_{i} \| \| \overline{\xiv}_i  \|)^2 }{4 (e^{2t} - 1)}, 
\]
\[
\sum_{|\alpha| = m } \| \zetav_i^{\alpha}\|^2 =   \frac{1}{(2 m!)^2 L^{l} (e^{2t} - 1)^{(m-l)}}  \| \xiv'_{i} - \xiv_{i} \|^2   \|  \overline{\xiv}_i \| ^{2 (m - l)}.  
\]Then setting $l = m - 1$ one gets 
\begin{equation*}
\sum_{\alpha \geq 0 }^{\infty}  \alpha ! (L-1)^{|\alpha|} \| \zetav_i^\alpha \|^2 \leq \frac{L}{e^{2t} -1} 
\left( \left(1 + \frac{e}{4} \right) \| \xiv'_{i} - \xiv_{i} \|^2  \|  \overline{\xiv}_i \|^2 + \frac{  (\E \| \xiv'_{i} - \xiv_{i} \|  \|  \overline{\xiv}_i \|)^2 }{4} \right).
\end{equation*}Apply expectation operator and make summation by $i$ 
\begin{equation}
\label{chast1}
 \left[  \sum_{i, \alpha}  \alpha ! (L-1)^{| \alpha |} \E \| \zetav_i^\alpha \|^2   \right]^{1/2} 
 \leq   \frac{(2L)^{1/2}}{(e^{2t} -1)^{1/2}} 
\left(  \sum_{i=1}^n \E \| \xiv'_{i} - \xiv_{i} \|^2  \|  \overline{\xiv}_i \|^2  \right)^{1/2}.
\end{equation}Analogical expression holds in power $L/2$:  
\begin{equation}\label{chast2}
\left[ \sum_i \E \left( \sum_{\alpha \geq 0}  \alpha! (L-1)^{|\alpha|} \| \zetav_i^\alpha \|^2  \right)^{L/2}  \right]^{1/L}
\leq   \frac{(2L)^{1/2}}{(e^{2t} -1)^{1/2}} 
\left(  \sum_{i=1}^n \E \| \xiv'_{i} - \xiv_{i}\|^{L}  \|  \overline{\xiv}_i \|^L  \right)^{1/L}.
\end{equation}For the other part of bound in Lemma \ref{Hsum} one has to evaluate term  $\| \sum_i \E \zetav_i^\alpha \|^2$. Note that 
\[
\sum_\alpha \left \| \sum_i \E \zetav_i^\alpha \right \|^2 = \sum_{i,j} \sum_\alpha  (\E \zetav_i^\alpha)^T \E X_j^\alpha  
\]
and $\forall l > 0$:
\[
\sum_{|\alpha| = 1 }   (\E \zetav_i^\alpha)^T \E X_j^\alpha   \leq  \frac{ \E \| \xiv'_{i} - \xiv_{i} \|  \|  \overline{\xiv}_i \|^{1 + l} \E \| \xiv'_{j} - \xiv_{j} \|  \|  \overline{\xiv}_i \|^{1 + l}     }{4} \frac{L^{l}}{(e^{2t} - 1)^{l+1}}  
\]and for $m >1$:
\[
\sum_{|\alpha| = m }   (\E \zetav_i^\alpha)^T \E X_j^\alpha \leq   \frac{
\E  \| \xiv'_{i} - \xiv_{i} \|  \|  \overline{\xiv}_i \| ^{ (m - l)} \E \| \xiv'_{j} - \xiv_{j} \|  \|  \overline{\xiv}_i \| ^{ (m - l)} 
}{(2 m!)^2 L^{l} (e^{2t} - 1)^{(m-l)}}.  
\]
Then setting $l = m - 2$ one obtains
\begin{equation}\label{chast3}
 \left[  \sum_{\alpha \geq 0}  \alpha! (L-1)^{|\alpha|}  \| \E \zetav^\alpha \|^2   \right]^{1/2} 
 \leq   \frac{e^{1/2} L}{e^{2t} -1} 
  \sum_{i=1}^n \E \| \xiv'_{i} - \xiv_{i} \|  \|  \overline{\xiv}_i \|^2.
 \end{equation}
Moreover, setting $l = m - 1$ we additionally derive that   \begin{equation}\label{chast4}
  \left[  \sum_{\alpha \geq 0}  \alpha! (L-1)^{|\alpha|}  \| \E \zetav^\alpha \|^2   \right]^{1/2} 
 \leq   \frac{e^{1/2} L^{1/2}}{(e^{2t} -1)^{1/2}} 
  \sum_{i=1}^n \E \| \xiv'_{i} - \xiv_{i}\|  \|  \overline{\xiv}_i \| 
  = \frac{ \| \Sigma \|^{1/2} \mu_2 e^{1/2} L^{1/2}}{(e^{2t} -1)^{1/2}}. 
 \end{equation}
 The last term requires two bounds because integration of function  $e^{-t}/(e^{2t} -1)$ diverges near zero point. We just have shown above in equation (\ref{phi_plus_tau}) that 
 \[
  \nabla \mathcal{G}_t(X_t)  = -e^{-t}  \sum_{i, \alpha} \zetav^\alpha_i H_\alpha(\gammav).
 \]
 From Lemma \ref{Hsum} and expressions (\ref{chast1}), (\ref{chast2}), (\ref{chast3}), (\ref{chast4}) follows that 
 \begin{align*}
 \frac{ \left[ \E \| \nabla \mathcal{G}_t(X_t) \|^L  \right]^{1/L} } {\| \Sigma \|^{1/2}} &\leq  \frac{C \, L^{3/2} e^{-t}}{\log(L) (e^{2t} -1)^{1/2}} \left( \mu_4^{1/2}  
 + \mu_{2L}^{1/L} \right) \\
 & + \min \left[  \frac{e^{1/2} L e^{-t}}{e^{2t} -1}  \mu_3, \,\,  \frac{ e^{1/2} L^{1/2} e^{-t}}{(e^{2t} -1)^{1/2}} \mu_2  \right].
 \end{align*}
 Now in order to obtain the bound for $W_L(\xiv, \gammav)$ by means of Lemma \ref{was_int_bound} one has to integrate the previous expression by $t$. Apply the following integrals:
\[
\int_0^{\infty} \frac{e^{-t}}{(e^{2t} -1)^{1/2}}dt  = 1 .
\]For $t_0 = 1/n$

\begin{align*}
& A \int_0^{t_0} \frac{e^{-t}}{(e^{2t} -1)^{1/2}}dt  + B \int_{t_0}^{\infty} \frac{e^{-t}}{e^{2t} -1}dt  \\
& = A(1 - e^{-2t_0})^{1/2}
+ B \left( -e^{-t_0} + \frac{1}{2} \log \frac{e^{-t_0} + 1}{ 1 - e^{-t_0}} \right) \\
& \leq \frac{\sqrt{2} A}{ \sqrt{n}} + \frac{B}{2} \log(2n).
\end{align*}
Set $A =  e^{1/2} L^{1/2} \mu_2$ and $B = e^{1/2} L \mu_3$, then finally
 \[
  \int_0^{\infty} \frac{ \left[ \E \|\nabla \mathcal{G}_t(X_t) \|^L  \right]^{1/L} }{\| \Sigma \|^{1/2}} dt \leq 
 \frac{C \, L^{3/2} }{\log L } \left( \mu_4^{1/2} + \mu_{2L}^{1/L} \right) 
 + \frac{ \sqrt{2}   e^{1/2} L^{1/2}  \mu_2 }{ \sqrt{n}} + \frac{ e^{1/2} L  \mu_3  }{2} \log(2n).
 \]
%  If all random variables $\xi_{ik}$ are sub-Gaussian with parameter $\nu$ as defined in the theorem, then one may use the following values for the moments (by means of Lemma \ref{sub_g_m})
%  \[
%  \mu^{1/L}_{2L} \leq   \mu^{1/2}_{4}  \leq \frac{ 4 \nu^2 e^{2/e} } {\sqrt{n}},
%  \quad
%  \mu_3 \leq  \frac{  \nu^3 e^{3/e} 3^{3/2} } {\sqrt{n}}
%  \]
\end{proof} 


\noindent Consider a random vector \(\xiv\) which has restricted exponential or sub-Gaussian moments: $ \exists \; \gm>0$
\begin{equation}
    \log \E \exp\bigl( \gammav^{\T}\xiv\bigr)
    \le
    \| \gammav \|^{2}/2,
    \quad
    \gammav \in \R^{\dimp}, \quad \| \gammav \| \le \gm 
\label{expgamgm}.
\end{equation}
For ease of presentation, assume below that \( \gm \) is sufficiently large.

% \input{subG.tex}


\begin{lemma}[\cite{spokoiny2017}]
\label{LLbrevelocro}   
Define $\xxc = \gm^{2}/4$.
Let \eqref{expgamgm} hold and 
\( 0.3 \gm \ge \sqrt{\dimp} \).
Then
%\( \E \|\xi\|^{2} \le \dimB \), and 
for each \( \xx > 0 \)
\[
    \P\bigl( \|\xiv\| \ge \zq(\dimp,\xx) \bigr)
    \leq
    2 \ex^{-\xx} + 8.4 \ex^{-\xxc } \Ind(\xx < \xxc) ,
\]   
where \( \zq(\dimp,\xx) \) is defined by
% with \( \xxc = \dimp \), \( \zqc = \sqrt{5 \dimp} \), and \( \gmc = \muc \zqc \) by
\[
\label{PzzxxpBro}
    \zq(\dimp,\xx)
     =  
    \begin{cases}
        \bigl( \dimp + 2 \sqrt{\dimp \xx} + 2 \xx\bigr)^{1/2}, &  \xx \le \xxc \\
        \gm + 2 \gm^{-1} (\xx - \xxc)   , & \xx > \xxc .
    \end{cases}
\]    
\end{lemma}

\begin{lemma}\label{subg_moments}

With conditions from Lemma \ref{LLbrevelocro} for each $k \geq 2$
\[
   \E \left \| \xiv  \right \|^k \leq 4 (\sqrt{p} + \sqrt{2k})^{k}.
\]
\end{lemma}

\begin{proof} First  separate events $\{  \| \xiv   \| \leq \sqrt{p}  \} $ and $\{  \| \xiv   \| > \sqrt{p}  \} $. Then we obtain
 \[
\E \| \xiv \|^k   \leq  p^{k/2} +  k \int_{\sqrt{p}}^{\infty} t^{k-1} \P (\| \xiv \| > t) dt. 
\]
Apply Lemma \ref{LLbrevelocro} that is valid in the region $\{  t > \sqrt{p}  \} $ 
\begin{align*}
&  \int_{\sqrt{p}}^{\infty} t^{k-1} \P (\| \xiv \| > t) dt \\
& \leq 2 \int_{0}^{\infty} z(p, \xx)^{k-1} (\ex^{-\xx}) z'(p, \xx) d\xx  \\
& + 8.4 e^{-\xxc} \int_{0}^{\xxc} z(p, \xx)^{k-1} d z(p, \xx).
\end{align*}Through integration by parts we find that 
\[
k \int_{0}^{\infty} z(p, \xx)^{k-1} (\ex^{-\xx}) z'(p, \xx) d\xx = -z^k(p, 0) + \int_{0}^{\infty} z(p, \xx)^{k} (\ex^{-\xx})  d\xx .
\]The function $z(p, \xx)$ behaves differently before and after the point $\xxc$.  So we will integrate it separately. 
\begin{align*}
& \int_{0}^{\xxc} z(p, \xx)^{k} (\ex^{-\xx})  d\xx  = \int_{0}^{\xxc} (\sqrt{p} + \sqrt{2x} )^{k} (\ex^{-\xx})  d\xx \\
& \leq \int_{0}^{\infty} (\sqrt{p} + y)^k e^{- \frac{y^2}{4}}  e^{-\frac{y^2}{4}} d \frac{y^2}{2} \\
& \leq \{ \text{set } y = \argmax (\sqrt{p} + y)^k e^{- \frac{y^2}{4}}  \} \leq \frac{  (\sqrt{p} + \sqrt{2k})^k }{2}  \int_{0}^{\infty}  e^{- \frac{y^2}{4}} d \frac{y^2}{2} \\
&  \leq   (\sqrt{p} + \sqrt{2k})^k  .
\end{align*}
\begin{align*}
& \int_{\xxc}^{\infty} z(p, \xx)^{k} (\ex^{-\xx})  d\xx  = \int_{\xxc}^{\infty} \left(g + \frac{2}{g} (\xx - \xxc) \right)^{k} (\ex^{-\xx})  d\xx \\
& = e^{-\xxc} \int_{0}^{\infty}   \left(g + \frac{2}{g} y \right)^{k} e^{-\frac{y}{2}} e^{-\frac{y}{2}} dy \\
& \leq \left \{  \left(g + \frac{2}{g} y \right)^{k} e^{-\frac{y}{2} } \leq \max  \left \{g, \frac{4k}{g}  \right\}^{k} \right \} \leq  2 e^{-\xxc}  \max \left\{ g,   \frac{4k}{g}  \right\}^k  \\
& \leq 2 e^{-k/2} (k)^{k/2}.
\end{align*}Compute the last integral part: 
\[
8.4 e^{-\xxc} k  \int_{0}^{\xxc} z(p, \xx)^{k-1} d z(p, \xx)  = 8.4 e^{-\xxc} (\sqrt{p} + \sqrt{2\xxc})^k \leq (\sqrt{p} + \sqrt{k})^k.
\]

% \begin{align*}
% &  \int_{\sqrt{p}}^{\infty} t^{q-1} \P (\| \xiv \| > t) dt \\
%  & \leq  \int_{0}^{\xxc} z(p, \xx)^{q-1} (2 \ex^{-\xx} + 8.4 \ex^{-\xxc })  z'(p, \xx) d\xx  \\
% & + \int_{\xxc}^{\infty} z(p, \xx)^{q-1} (2 \ex^{-\xx}) z'(p, \xx) d\xx 
% \end{align*}


\end{proof}


\noindent Using the last lemma one may evaluate moments in Theorem \ref{WLT}. 

\begin{theorem} \label{WLTsubG} Under conditions from Theorem \ref{WLT} and additional condition that $ \forall i: \, \frac{\sqrt{n}}{\nunu} \Sigma^{-1/2} \xiv_i $ is sub-Gaussian (\ref{expgamgm})

\[
W_L(\xiv, \gammav) \leq 
\frac{C \, L^{3/2} \nunu^2 \| \Sigma \|^{1/2} }{\log L } \left( \frac{p}{\sqrt{n}} + \frac{L}{n^{1 - 1/L}} \right)  +  \frac{5 L \nunu^3 p^{3/2} \| \Sigma \|^{1/2} \log(2n) }{\sqrt{n}},
\] for some absolute constant $C$.


\end{theorem}

\begin{remark} The main advantage of this theorem is explicit and sharp dependence on parameters $n$, $p$ and $L$.  
 A simplified asymptotic of this upper bound is 
\[
O\left( \frac{ L^{3/2} p + L p^{3/2} \log n }{\sqrt{n}} \right).
\]
Compare the last result with Lemma \ref{was_1d} in one dimensional case ($p=1$). The asymptotic by $L$ is the same or better depending on the distribution of $\xi$.
This bound remains sharp in case $L = 1$ and comparable with results of \cite{Bentkus, buzun2019gaussian} that studies Gaussian approximation in $W_1$.  
\end{remark}


==> bernulli2020(4)/main_res.tex <==

 In this work, we prove the Theorem that finds the upper bound for the strong Gaussian approximation. Herein, we consider a sum of independent zero-mean random vectors $\xiv = \sum_{i=1}^n \xiv_i$ in $\R^{p}$ that has a covariance matrix 
$$
\Sigma = \E \xiv \xiv^T.
$$
A Gaussian random vector $\gammav \in \ND(0, \Sigma)$ has the same 1-st and the 2-nd moments. 
% Assume that the indices $i \in {1, \ldots, n}$ correspond to the elements in the sum and the indices $k \in {1, \ldots, p} $ correspond to the components of the vector $\xiv$. 
 We say that a vector \(\xiv\) has restricted exponential or sub-Gaussian moments if $ \exists \; \gm>0$
\begin{equation}
    \log \E \exp\bigl( \lambdav^{\T}\xiv\bigr)
    \le
     \| \lambdav \|^{2}/2,
    \quad
    \forall \lambdav \in \R^{\dimp}, \quad \| \lambdav \| \le \gm 
\label{expgamgm_2}.
\end{equation}

\begin{theorem} \label{main_res} Under condition that $ \forall i: \, \frac{\sqrt{n}}{\nunu} \Sigma^{-1/2} \xiv_i $ is sub-Gaussian (expression (\ref{expgamgm_2}) with \( 0.3 \gm \ge \sqrt{\dimp} \)) exists a Gaussian vector $ \gammav \in \ND (0, \Sigma)$ such that 

\[
\P \left(  \left \|   \xiv -  \gammav \right\| > C(n, p) \|\Sigma \|^{1/2} \, e^{t/\log(np)} \right) \leq
e^{-t},
\]
where 
\[
C(n, p) =  C \,  \nunu^2 \,   \frac{p \log(np)^{3/2} }{\sqrt{n}}  +  5 \nunu^3 \, \frac{  p^{3/2} \log(np) \log(2n) }{\sqrt{n}},
\] for some absolute constant $C$.


\end{theorem}


\noindent \emph{Summary of the proof:} Our approach is based on the optimal transport theory \cite{OttoVillani, BobkovEd, Bonis}. It consists of the following steps. 

\begin{itemize}
 \item A very useful tool in  approximation in probability is the Wasserstein distance (expression \ref{equation_3}). It reveals the joint distribution and minimises the difference between two random variables by increasing their dependence with some fixed marginal distributions.   The multivariate Central Limit Theorem for $W_2$ distance was described by \cite{Bonis}, where the author 
 uses Stein's method and the entropy estimation for the derivative of $W_2$.  Below, basing on the same technique, we obtain Gaussian approximation bound for $W_L$ with explicit dependence on the power $L$ of the cost function and dimension parameter $p$ (Theorem \ref{WLTsubG}), such that 
\[
W_L(\xiv, \gammav) \leq 
\frac{C \, L^{3/2} \nunu^2 \| \Sigma \|^{1/2} }{\log L } \left( \frac{p}{\sqrt{n}} + \frac{L}{n^{1 - 1/L}} \right)  +  \frac{5 L \nunu^3 p^{3/2} \| \Sigma \|^{1/2} \log(2n) }{\sqrt{n}}.
\]
The proof of the last statement is the most difficult part of this work. It starts with derivative estimation of $W_L$.  For that we construct a Markov random process $X_t$ that transits $X_0 = \xiv$ to $X_\infty = \gammav$. From Lemma \ref{was_int_bound} follows that for the random process $X_t$ under smoothness condition it holds  \[
W_L(X_a, X_b) \leq
\int_{a}^{b}  \left\{ \E \left \|  \E \left[ \frac{d}{dt} X_t \bigg | X_t \right] \right \|^L  
\right \}^{1/L} dt .
\]Then in order to derive an upper bound for $\E \left \|  \E \left[ \frac{d}{dt} X_t  | X_t \right] \right \|^L  $ we involve Rosenthal's martingale inequality (Lemma \ref{rose}), convolution with Hermite polynomials (Lemma \ref{boni}), and modified variant of  Stein's method (Theorem \ref{WLT}).    
\item The sub-Gaussian property is required for moments estimation of random variables $\|\xiv_i \|$ (used in Theorem \ref{WLT}) and in Lemma \ref{subg_moments} we have proved the following upper bound for each $k \geq 2$ and $1 \leq i \leq n$
\[
   \E \left \| \Sigma^{-1/2} \xiv_i  \right \|^k \leq \frac{4 \nunu^k}{n^{k/2}} (\sqrt{p} + \sqrt{2k})^{k}.
\]
\item Denote a joint distribution of $\xiv$ and $\gammav$ by $\pi = \pi(\xiv, \gammav)$.   Markov's inequality provides the following statement \[ 
\min_{\pi \in \Pi[\xiv, \gammav]} \P \left(   \normx{\xiv - \gammav} > \Delta \right) \leq  \frac{W_L^L(\xiv, \gammav)} {\Delta^L}, 
\]
where we set $L = \log (np)$ and $\Delta = C(n, p) \| \Sigma \|^{1/2} \, e^{t/\log(np)}$.


\end{itemize}


\begin{remark}
Note that convergence in probability in Central Limit Theorem does not exist, \textit{i.e.}, there is no random vector $ \gammav$, such that $\xiv(n)$ converges to it when $n \to \infty$. It follows from the Kolmogorov's  $0$-$1$ law. However, at the same time, for each $n$ one should take a new Gaussian vector which depends on $n$ and 
\[
 \| \xiv (n) - \gammav (n) \| \overset{p}{\longrightarrow} 0,
\quad 
n \to \infty,
\]
which follows from Theorem \ref{main_res}.
\end{remark}

==> bernulli2020(4)/mydef.tex <==
%\renewcommand{\)}{\,\end{math}}
\renewcommand{\(}{$\,}
\renewcommand{\)}{\,$}

\def\Fbb{\mathbb{F}}
\def\Ftt{\mathbb{F}_{\theta }}
\def\Fee{\mathbb{F}_{\eta }}
\def\Fttv{\mathbb{F}_{\vartheta }}
\def\Fuu{\mathbb{F}_{u }}
\def\Fte{\mathbb{F}_{\theta \eta }}
\def\Fet{\mathbb{F}_{\eta \theta}}

\def\ub{u^{\flat}}

\newcommand{\normx}[1]{\left \|#1 \right \|}
\newcommand{\normX}[1]{\left \|#1 \right \|}

\def\rr{\mathtt{r}}
\def\rrb{\rr^{*}}
\def\rru{\rr_{\circ}}
\def\rrc{\rr'}
\def\rs{r_{*}}

\def\zz{\mathfrak{z}}
\def\zzb{\tilde{\zz}}
\def\tt{\mathfrak{t}}
\def\zb{z_{\rd}}
\def\zzg{\zz_{1}}
\def\zzQ{\zz_{0}}
\def\zzq{\zz}

\def\rombb{\diamondsuit^{\flat}(r,x)}
\def\romb{\diamondsuit(r,x)}
\def\rombproj{\diamondsuit_{\vartheta}(\rr,x)}

\def\gaussv{\gamma}
\def\gauss{\varepsilon}

\def\gpsii{g(\psi_i^{T} \theta)}
\def\gpsiidev{g''(\psi_i^{T} \theta)}
\def\rb0{r_0^{\flat}}

\def\nquad{\hspace{-1cm}}
\def\eqdef{\stackrel{\operatorname{def}}{=}}
\def\tod{\stackrel{d}{\longrightarrow}}
\def\tow{\stackrel{w}{\longrightarrow}}
\def\toP{\stackrel{\P}{\longrightarrow}}
\def\epsb{\varepsilon^{\flat}}

\def\bX{X^{\flat}}
\def\bXT{X^{\flat T}}

\def\tS{\tilde{S}}
\def\Sv{\bf{S}}
\def\xiv{\bf{\xi}}
\def\tXv{\tilde{\Xv}}
\def\tX{\tilde{X}}
\def\tY{{\widetilde{Y}}}
\def\GFC{\cc{G}_{3}}
\def\bdelta{\delta^{\sbt}}
\def\bqq{\qq^{\sbt}}
\def\tdelta{\err}%{\tilde{\delta}}
\def\tqq{\tilde{\qq}}
\def\eps{\varepsilon}
\def\fs{f}
\def\vp{\mathrm{v}}
\def\CONST{C}
\def\teps{\tilde{\varepsilon}}
\def\ND{\mathcal{N}}
\def\Ybb{\mathbb{Y}}

\def\dLhSeq{\mathbb{T}_h}
\def\dLhConv{\text{TP}_h}
\def\YL{\mathbb{Y}_L}
\def\YR{\mathbb{Y}_R}
\def\YLL{Y_{t-h},\ldots, Y_{t - 1}}
\def\YRR{Y_{t},\ldots, Y_{t + h - 1}}

\newcommand{\cc}[1]{\mathscr{#1}}
%\newcommand{\cc}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\boldsymbol{#1}}

%\renewcommand{\bar}[1]{\overset{\!\_\!\_\!\_}{#1}}
\renewcommand{\bar}[1]{\overline{#1}}
\renewcommand{\hat}[1]{\widehat{#1}}
\renewcommand{\tilde}[1]{\widetilde{#1}}


\renewcommand{\Gamma}{\varGamma}
\renewcommand{\Pi}{\varPi}
\renewcommand{\Sigma}{\varSigma}
\renewcommand{\Delta}{\varDelta}
\renewcommand{\Lambda}{\varLambda}
\renewcommand{\Psi}{\varPsi}
\renewcommand{\Phi}{\varPhi}
\renewcommand{\Theta}{\varTheta}
\renewcommand{\Omega}{\varOmega}
\renewcommand{\Xi}{\varXi}
\renewcommand{\Upsilon}{\varUpsilon}
%
\def\nn{\nonumber \\}

\def\suml{\sum\limits}
\def\supl{\sup\limits}
\def\maxl{\max\limits}
\def\infl{\inf\limits}
\def\intl{\int\limits}
\def\liml{\lim\limits}
\def\Cov{\operatorname{Cov}}
\def\Var{\operatorname{Var}}
\def\arginf{\operatornamewithlimits{arginf}}
\def\argsup{\operatornamewithlimits{argsup}}
\def\argmax{\operatornamewithlimits{argmax}}
\def\argmin{\operatornamewithlimits{argmin}}
\def\val{\operatorname{val}}

%\def\E{\boldsymbol{E}}
%\def\P{\boldsymbol{P}}
\def\D{\boldsymbol{D}}
\def\dd{\operatorname{d}}
\def\tr{\operatorname{tr}}
\def\I{I\!\!I}
\def\R{I\!\!R}
\def\E{I\!\!E}
\def\P{I\!\!P}
\def\X{\mathfrak{X}}
\def\kappa{\varkappa}
%\def\R{\mathbb{R}}
\def\Const{\mathrm{Const.} \,}
\def\cdt{\boldsymbol{\cdot}}
\def\tm{\!\times\!}
\def\T{\top}
\def\diag{\operatorname{diag}}
\def\bldiag{\operatorname{blockDiag}}
\def\diam{\operatorname{diam}}
\def\rank{\operatorname{rank}}
\def\loc{\operatorname{loc}}

\def\tX{\widetilde{X}}
\def\txi{\widetilde{\xi}}
\def\teps{\widetilde{\varepsilon}}
\def\gtr{g_\triangle}

\def\nablaGLM{S}
\def\GLMLINK{A}
\def\GLMlink{g}
\def\aexpzeta{a}
\def\upsi{\upsilon}
\def\aGLMlink{a_g}


\def\av{\bb{a}}
\def\bv{\bb{b}}
\def\cv{\bb{c}}
\def\dv{\bb{d}}
\def\ev{\bb{e}}
\def\fv{\bb{f}}
\def\gv{\bb{g}}
\def\hv{\bb{h}}
\def\iv{\bb{i}}
\def\jv{\bb{j}}
\def\kv{\bb{k}}
\def\lv{\bb{l}}
\def\mv{\bb{m}}
\def\nv{\bb{n}}
\def\ov{\bb{o}}
\def\pv{\bb{p}}
\def\qv{\bb{q}}
\def\rv{\bb{r}}
\def\sv{\bb{s}}
\def\tv{\bb{t}}
\def\uv{\bb{u}}
\def\vv{\bb{v}}
\def\wv{\bb{w}}
\def\xv{\bb{x}}
\def\yv{\bb{y}}
\def\zv{\bb{z}}

\def\Cv{\bb{C}}
\def\Gv{\bb{G}}
\def\Mv{\bb{M}}
\def\Sv{\bb{S}}
\def\Uv{\bb{U}}
\def\Xv{\bb{X}}
\def\Yv{\bb{Y}}
\def\Zv{\bb{Z}}


\def\alphav{\bb{\alpha}}
\def\betav{\bb{\beta}}
\def\gammav{\bb{\gamma}}
\def\deltav{\bb{\delta}}
\def\varepsilonv{\bb{\varepsilon}}
\def\epsv{\bb{\varepsilon}}
\def\etav{\bb{\eta}}
\def\gammav{\bb{\gamma}}
\def\phiv{\bb{\phi}}
\def\psiv{\bb{\psi}}
\def\tauv{\bb{\tau}}
\def\upsilonv{\bb{\upsilon}}
\def\xiv{\bb{\xi}}
\def\zetav{\bb{\zeta}}

\def\Psiv{\bb{\Psi}}
\def\CONST{\mathtt{C}}

\def\dL{T}
\def\dLh{T_h}
\def\dLhb{T_h^{\flat}}
\def\dLb12{T_h^{\flat}(\theta_1^{\flat}, \theta_2^{\flat})}
\def\dLht{T_h(t)}
\def\dLhconv{\text{TP}_h(\tau)}
\def\dLhconvb{\text{TP}_h^{\flat}(\tau)}
\def\dLhconve{\text{TP}_h^{\epsilon}(\tau)}
\def\dxi{\xi_{12}}
\def\dxib{\xi^{\flat}_{12}}
\def\dtheta{\theta_{12}^*}
\def\dthetahat{\widehat{\theta}_{12}}
\def\localr{\Theta(\rr)}
\def\gradL{\nabla L}

\def\thetab{\theta^{\flat}}
\def\opttheta{\widehat{\theta}}
\def\opteta{\widehat{\eta}}

\def\txi{\tilde{\xi}}
\def\txib{\tilde{\xi}^{\flat}}

\def\rombb{\diamondsuit^{\flat}(\rr,\xx)}
\def\romb{\diamondsuit(\rr,\xx)}
\def\rombe{\diamondsuit^{\epsilon}(\rr,\xx)}

\def\mle{\widehat{\theta}}
\def\reftheta{\theta^*}
\def\diagPsi{D(\Psi)}

\def\alphab{\alpha^{\flat}}
\def\chb{\chi^{\flat}}
\def\alphab12{\alpha^{\flat}(\theta, \theta_0)}
\def\chib12{\chi^{\flat}(\theta, \theta_0)}
\def\Lbf{L^{\flat}(\theta)}
\def\Lb0{L^{\flat}(\theta_0)}
\def\Lbopt{L^{\flat}(\widehat{\theta})}
\def\Lfopt{L(\widehat{\theta})}
\def\Lf{L(\theta)}
\def\L0{L(\theta_0)}

\def\Eb{\E^{\flat}}
\def\Varb{\Var^{\flat}}

\def\itemv{\vfill\item}
\newenvironment{myslide}[1]
    {\begin{frame}\frametitle{#1}\vfill}
    {\vfill\end{frame}}

\def\vsp{\vspace{0.05\textheight} \vfill}
\def\summarysign{\resizebox{0.08\textwidth}{0.08\textheight}{\includegraphics{summary}}\,}
\def\nix{}
\def\wpu{$\bullet$}

\def\btri{\vfill{\( \blacktriangleright \) }}
\def\btrir{\vfill{\( \blacktriangleright \) }}

\newcommand{\mygraphics}[3]{\begin{center}
    \resizebox{#1\textwidth}{#2\textheight}{\includegraphics{#3}}
    \end{center}
}

\newcommand{\mybox}[3]{\begin{center}
    \resizebox{#1\textwidth}{#2\textheight}{#3}
    \end{center}
}
\newcommand{\tobedone}[1]{\par\textbf{\color{red}To be done:} {\color{magenta}#1}}
\def\tobechecked{\qquad{\color{red} \text{\( (^{*}) \) please check}}}

%\definecolor{myhcolor}{rgb}{0.2,0,0.8}
%\definecolor{myhcolor}{named}{red}
\newenvironment{eqnh}
{
    %\color{myhcolor}} {}
    \setbeamercolor{postit}{fg=black,bg=hellgelb} %{fg=myhcolor,bg=white}
    \begin{beamercolorbox}[center,wd=\textwidth]{postit} %rounded=true,shadow=true,
    \begin{eqnarray*}}
    {\end{eqnarray*}\end{beamercolorbox}
}


\newcommand{\normp}[1]{
\left\Vert #1 \right\Vert
}

\newcommand{\normop}[1]{
\left\Vert #1 \right\Vert_{\oper}
}

\newcommand{\pr}[1]{
\P\left( #1 \right)
}

\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}


\def\Bernoulli{\mathrm{Bernoulli}}
\def\Vola{\mathrm{Vola}}
\def\Poisson{\mathrm{Poisson}}
\def\ag{\mathrm{ag}}
\def\glob{\operatorname{glob}}
\def\lin{\operatorname{lin}}
\def\cond{\, \big| \,}

\def\rdl{\epsilon}
\def\rd{\bb{\rdl}}
\def\rddelta{\delta}
\def\rdomega{\varrho}
\def\rddeltab{\rddelta^{*}}
\def\rhorb{\rhor^{*}}




\def\wv{\bb{w}}
\def\varthetav{\bb{\vartheta}}
\def\Lr{\breve{L}}
\def\zetavr{\breve{\zetav}}
\def\etavr{\breve{\etav}}
\def\xivr{\breve{\xiv}}


\def\rdb{\rd}
%\def\rdm{\bb{\sigma}}
\def\rdm{\underline{\rdb}}

\def\taub{\tau_{\rdb}}
\def\taum{\tau_{\rdm}}
\def\kappab{\kappa_{\rd}}
\def\deltab{\delta_{\rd}}

\def\taubGP{\tau_{\rdb,\GP}}
\def\taumGP{\tau_{\rdm,\GP}}
\def\kappabGP{\kappa_{\rd,\GP}}
\def\deltabGP{\delta_{\rd,\GP}}
\def\nubm{\nu_{\rd}}
\def\uub{u_{\rd}}
\def\uubGP{u_{\rd,\GP}}
\def\nubmGP{\nu_{\rd, G}}


\def\rG{\rd,\GP}

\def\LinSp{\mathrm{L}}
\def\Id{I\!\!\!I}
\def\Ind{\operatorname{1}\hspace{-4.3pt}\operatorname{I}}

\def\BG{\mathcal{R}}
\def\bg{r}
\def\fmup{\phi}
\def\rg{r}
\def\uc{u_{c}}
\def\muc{\mu_{c}}
\def\mud{\mu_{0}}
\def\xxd{\xx_{0}}
\def\yyd{\yy_{0}}
\def\gmd{\gm_{0}}

\def\ms{m^{*}}
\def\Inv{A}
\def\InvT{\Inv^{\T}}
\def\Invt{\tilde{\Inv}}


\def\ssize{N}
\def\nsize{{n}}

%\def\rhor{\mathfrak{b}}
\def\rhor{\omega}


\def\LT{L}
\def\LGP{\LT_{\GP}}
%\def\La{\breve{L}}
\def\La{\mathbb{L}}
\def\Lab{\La_{\rdb}}
\def\Lam{\La_{\rdm}}

\def\DP{D}
\def\DPc{\DP_{0}}
\def\DPb{\DP_{\rdb}}
\def\DPm{\DP_{\rdm}}

\def\LabGP{\La_{\rdb,\GP}}
\def\LamGP{\La_{\rdm,\GP}}

\def\DPbGP{\DP_{\rdb,\GP}}
\def\DPmGP{\DP_{\rdm,\GP}}
\def\riskbGP{\riskt_{\rdb,\GP}}

\def\gmi{\mathtt{b}}
\def\gmiid{\mathtt{g}_{1}}
\def\kullbi{\Bbbk}
\def\Thetasi{\Theta}
\def\rri{\mathtt{u}}
\def\rris{\rri_{0}}

\def\Ipc{\bb{\mathrm{f}}}
%\def\IF{\bb{\mathrm{f}}}
\def\IF{\Bbb{F}}
\def\IFc{\IF_{0}}
\def\IFb{\IF_{\rdb}}
\def\IFm{\IF_{\rdm}}


\def\DF{\cc{D}}
\def\DFc{\DF_{0}}
\def\DFb{\DF_{\rdb}}
\def\DFm{\breve{\DF}_{\rd}}
\def\DFm{\DF_{\rdm}}

\def\DPr{\breve{\DP}}
\def\VF{\cc{V}}
\def\VFc{\VF_{0}}

\def\HHc{\HH_{0}}
\def\HHb{\HH_{\rd}}
\def\HHm{\HH_{\rdm}}


\def\xib{\xiv^{\flat}}
\def\xivb{\xiv_{\rdb}}
\def\xivm{\xiv_{\rdm}}
\def\CAm{\underline{\CA}}
\def\CAb{\CA}

\def\penr{\operatorname{pen}}
\def\pen{\mathfrak{t}}
\def\PEN{\operatorname{PEN}}
\def\RSS{\operatorname{RSS}}
\def\med{\operatorname{med}}

\def\ex{\mathrm{e}}
%\def\bracketing{\diamond}
\def\entrl{\mathbb{Q}}
%\def\entrlr{\mathbb{Q}^{\bracketing}}
\def\entrlb{\entrl}
%\def\entrlp{\entrl_{p}^{*}(\mrho)}
%\def\entrlq{\entrl_{p}^{*}(\qqq)}
%\def\entrlG{\entrl(\GV)}
\def\entr{\entrl}

\def\kullb{\cc{K}} %{\wp}
\def\kullbc{\kullb^{c}}


\def\gm{\mathtt{g}}
\def\gmc{\gm_{c}}
\def\gmb{\gm}
\def\gmbm{\gmb_{1}}

\def\yy{\mathtt{y}}
\def\yyc{\yy_{c}}
%\def\yyn{\yy_{0}}
\def\xx{\mathtt{x}}
\def\xxc{\xx_{c}}
\def\tc{t_{c}}

\def\alp{\alpha}
\def\alpn{\rho}
%\def\as{a_{0}}
%\def\daas{\Phi}
\def\gmu{\mathfrak{a}}


\def\losst{\varrho}
\def\loss{\wp}
\def\lossp{u}
\def\closs{g}

\def\riskt{\cc{R}}
\def\emprisk{\ell}
\def\bias{b}
\def\biasv{\bb{b}}
\def\bern{q}

%\def\nuu{\mathfrak{u}}
%\def\nud{\mathfrak{u}_{0}}
%\def\nun{c_{\nuu}}



\def\TT{\nsize}

\def\Pone{P}
%\def\Ef{\E}
%\def\Pf{\P}
\def\Pf{\P_{f(\cdot)}}
\def\Ef{\E_{f(\cdot)}}
\def\Ps{\P_{\thetas}}
\def\Es{\E_{\thetas}}
\def\Pu{\P_{\upsilons}}
\def\Eu{\E_{\upsilons}}

\def\Pvs{\P_{\thetavs}}
\def\Evs{\E_{\thetavs}}

%\def\upsdc{\ups_{0}}
\def\UPd{w}
\def\nunup{\nu_{1}}
\def\rru{\rr_{1}}
\def\rups{\rr_{0}}
\def\rupsb{\rups^{*}}
\def\rrf{\rr^{\flat}}
\def\rupd{\rr_{\circ}}


\def\smooths{\mathbb{S}}
\def\smooth{\smooths_{1}}


\def\elli{\bar{\ell}}


%\def\Pu{Q}

\def\K{K}

\def\Psir{\breve{\Psi}}

\def\af{a}
\def\afs{\af^{*}}

\def\kapla{\varkappa}

\newcommand{\mlew}[1]{\tilde{\thetav}_{#1}}
\newcommand{\mlea}[1]{\hat{\thetav}_{#1}}
\newcommand{\mluw}[1]{\tilde{\theta}_{#1}}
\newcommand{\mlua}[1]{\hat{\theta}_{#1}}
\newcommand{\penm}[1]{\boldsymbol{m}_{#1}}

\def\Pdom{\mu_{0}}
\def\PDOM{\bb{\mu}_{0}}
\def\EDOM{\E_{0}}

\def\mk{m}
\def\Mk{\cc{M}}
\def\SV{\cc{S}}

\def\Cs{E}
\def\Csd{\Cs^{\circ}}
\def\Ca{A}
\def\CS{\cc{E}}
\def\CA{\cc{A}}
\def\CAb{\CA_{\rd}}
\def\CAC{\CA_{\CoFu}}

\def\Ccb{m_{\rdb}}
\def\Ccm{m_{\rdm}}
\def\CcbGP{m_{\rdb,\GP}}
\def\CcmGP{m_{\rdm,\GP}}

\def\etas{\eta^{*}}

\def\omegav{\bb{\phi}}
\def\omegavs{\omegav^{*}}
\def\omegavc{\omegav'}

\def\nuvs{\nuv^{*}}
\def\nuvc{\nuv'}

\def\nunu{\nu_{0}}
\def\numu{\nu_{1}}
%\def\nubu{\nu_{2}}
\def\nupi{\nu^{+}}
\def\nubu{\beta}

\def\nus{\nu}
\def\nusb{\nus}
\def\nusr{\nus^{\bracketing}}
\def\Nusb{\mathbb{N}}
\def\Nusr{\mathbb{N}^{\diamond}}

\def\dist{d}
\def\distd{\mathfrak{a}}

\def\hatk{\kappa}
\def\ko{k^{\circ}}


%\def\qq{\mathfrak{q}}
\def\qqq{\mathfrak{q}}
%\def\ppp{\mathfrak{s}}
\def\ppp{{s}}
\def\Cqq{C(\qqq)}
\def\Cqqb{C^{\diamond}(\qqq)}
%\def\Cqq{\qqq \log(2 \ppp)}
\def\Crho{C(\mrho)}
\def\Cqqm{\log(4)}
\def\Cqpr{(\qqq \rrp + \dimp / 2)}

\def\Cdima{\mathfrak{e}_{0}}
\def\Cdimb{\mathfrak{e}_{1}}
\def\cdima{\mathfrak{c}_{0}}
\def\cdimb{\mathfrak{c}_{1}}
\def\cdim{\mathfrak{c}}

\def\rdomega{\varrho}
\def\deltaD{\delta}
\def\alphai{\alpha_{1}}
\def\alphaii{\alpha_{2}}
\def\alphaiii{\alpha_{3}}
\def\alphaiv{\alpha_{4}}

\def\err{\diamondsuit}
%\def\rd{\varrho}
%\def\errb{\err_{\rdomega}}
\def\errbm{\bar{\err}_{\rdomega}}
\def\errm{\err_{\rdm}}
\def\errb{\err_{\rdb}}


\def\errbGP{\err_{\rdomega,\GP}}
\def\errmGP{\err_{\rdm,\GP}}
\def\errbmGP{\bar{\err}_{\rd,\GP}}

\def\errs{\err_{\rdomega}^{*}}
\def\deltas{\alpha}

\def\xivbGP{\xiv_{\rdb,\GP}}
\def\xivmGP{\xiv_{\rdm,\GP}}


\def\SP{S}
\def\GP{G}
\def\GPt{\GP_{0}}
\def\GPn{\GP_{1}}
\def\gp{g}
\def\gs{s}

%\def\SP{G}

\def\errbGP{\err_{\rdb,\GP}}
\def\errmGP{\err_{\rdm,\GP}}
\def\errpmGP{\err_{\GP}^{\pm}}
%\def\errsGP{\err_{\GP}^{*}}
%\def\deltaDGP{\delta_{\GP}}

\def\LCS{\cc{C}}

\def\DPGP{\DP_{\GP}}
\def\thetavsGP{\thetavs_{\GP}}


\def\LL{\cc{L}}
\def\LLb{\LL^{*}}
\def\LLh{\cc{L}}

\def\YY{\cc{Y}}
\def\LP{L^{\circ}}


\def\modcnrd{\mathfrak{A}}

\def\pens{\pi}
\def\pnn{\mathfrak{g}}
\def\pnnd{\mathfrak{u}}
%\def\pnnd{b}
\def\pnndGP{\pnnd_{\GP}}


\def\confpr{\mathfrak{c}}
\def\confprb{\confpr^{*}}

\def\pn{\pens^{*}}
\def\penInt{\mathfrak{D}}
\def\penH{\mathbb{H}}
\def\pmu{\mathfrak{u}}
\def\Closs{\cc{R}}

\def\dimp{p}
\def\riskb{\riskt_{\rdb}}
%\def\dimpp{\mathfrak{p}}
\def\dimpp{\dimp+1}
\def\BB{I\!\!B}
\def\vA{\mathtt{v}}


\def\deficiency{\Delta}
\def\spread{\Delta}
\def\dimtotal{\dimp^{*}}

\def\thetav{\bb{\theta}}
%\def\thetavs{\thetav_{0}}
\def\thetavs{\thetav^{*}}
\def\thetavc{\thetav'}
\def\thetavd{\thetav^{\circ}}
\def\thetavdc{\thetav^{\sharp}}
%\def\dthetavs{\thetav,\thetavs}
%\def\dthetavc{\thetav,\thetavc}
%\def\dthetavd{\thetav,\thetavd}
\def\dthetavs{\thetav,\thetavs}

\def\thetas{\theta^{*}}
\def\thetac{\theta'}
\def\thetad{\theta^{\circ}}

\def\thetavb{\thetav^{\dag}}

\def\vtheta{\vartheta}
\def\vthetav{\bb{\vtheta}}
%\def\prior{\operatorname{pr}}
\def\prior{\Pi}

\def\Gam{\Xi}
\def\Gam{\mathcal{S}}
\def\RG{R}
\def\Psu{\Upsilon}
\def\Phim{\breve{\Phi}}

\def\Proj{P}

\def\gammavs{\gammav^{*}}
\def\gammavd{\gammav^{\circ}}
\def\etavs{\etav^{*}}
\def\etavd{\etav^{\circ}}
\def\etavc{\etav'}

\def\taus{\tau_{0}}
\def\taup{\lceil \tau \rceil}

%\def\Sigmas{{\Sigma^{*}}}
\def\sigmas{{\sigma^{*}}}
\def\Sigmas{\Sigma_{0}}

\def\upsilonc{\upsilon'}
\def\upsilond{\upsilon^{\circ}}
\def\upsilonp{{\upsilon}^{*}}
\def\upsilonm{{\upsilon}_{*}}
\def\upsilonvs{\upsilonv^{*}}
\def\upsilons{\upsilon^{*}}
\def\upsilonb{\bar{\upsilon}}
\def\upsilonvd{\upsilonv^{\circ}}

\def\ups{\bb{\upsilon}}
%\def\upss{\ups_{0}}
\def\upsc{\ups^{\prime}}
\def\upsd{\ups^{\circ}}
%\def\upsd{\mathring{\ups}}
%\def\upsd{\breve{\ups}}
\def\upsdc{\ups^{\sharp}}
\def\upsdu{\ups^{\flat}}
\def\upss{\ups^{*}}
\def\upsr{\breve{\ups}}

\def\Ups{\varUpsilon}
\def\Upsd{\Ups^{\circ}}
\def\Upss{\Ups_{\circ}}
\def\UpsP{\Ups^{c}}

\def\Thetas{\Theta}
\def\ThetasGP{\Theta_{0,\GP}}
\def\varthetav{\bb{\vartheta}}


\def\glink{g}


\def\fvs{\fv}
\def\fs{f}
\def\fb{\fv^{\dag}}



%\def\uu{\bb{u}}
\def\uc{\uv'}
\def\ud{\uv^{\circ}}
\def\uvs{\uv^{*}}
\def\us{u^{*}}
\def\vs{v^{*}}


\def\reps{\epsilon}
\def\eps{\epsilon}

\def\repsc{\reps_{0}}
\def\repsb{\reps^{*}}
%\def\repsg{\mathfrak{e}}
\def\repsg{g}

\def\lu{\delta}
\def\lub{\bar{\lu}}

\def\Uu{U}
\def\UU{\cc{Y}}
\def\UUM{\cc{M}}
\def\UP{\cc{U}}
\def\up{\mathfrak{u}}

\def\VP{V}
\def\VPc{\VP_{0}}
\def\VPV{\cc{U}}
\def\VPVc{\cc{\VPV}_{0}}
\def\VPGP{\VP_{\GP}}
\def\VPSP{\VP_{\SP}}

\def\VV{H}
\def\GV{\cc{G}}
\def\GVS{S}

\def\VVb{\VV^{*}}
\def\VVc{\VV_{0}}
\def\vv{\bb{v}}
\def\vva{g}
\def\vp{\mathbf{v}}
\def\vpc{\vp_{0}}
\def\VVca{\VV}
\def\Vtt{H}


\def\DG{D}


\def\Vn{V_{0}}
\def\vn{v_{0}}

\def\norm{\mathfrak{c}}
%\def\normc{\mathfrak{d}}
\def\normc{\delta}
\def\norma{c}

\def\egridd{\cc{E}_{\delta}}
\def\penb{\varkappa}

\def\dotzeta{\dot{\zeta}}
%\def\mes{\operatorname{mes}}
\def\mes{\pi}
\def\mesl{\Lambda}
\def\cprr{F}

%\def\lambdab{\bar{\lambda}}
\def\lambdam{\gm_{1}}
\def\lambdaB{{\lambda}^{*}}
\def\lambdac{{\lambda'}}

%\def\cla{\mathfrak{b}}
\def\cla{{b}}
\def\fis{\mathfrak{a}}
\def\fiss{\fis_{1}}

\def\Vd{{V}}
\def\vd{\bar{v}}

\def\klim{k^{\circ}}
\def\midm{\mid \!}

\def\Ldrift{M}
\def\ldrift{m}
\def\mY{b}
\def\Lvar{D}
\def\lvar{\sigma}

\def\Mubcu{\Upsilon}
\def\Dthetav{\bb{u}}


\def\B{\cc{B}}
%\def\BD{\mathring{\B}}
\def\BD{\B^{\circ}}
\def\BU{B}
\def\BI{\B^{*}}
%\def\dD{d^{*}}

%\def\Ns{\mathbb{N}}
%\def\Nsd{\mathbb{N}_{\thetavd}}

\def\mub{\mu^{*}}
\def\mubc{\mu}
\def\mubcb{\mubc^{*}}
\def\Mubc{\mathbb{M}}
\def\Mubcb{\mathrm{M}}

\def\zzc{\zz_{c}}
\def\ww{w}
\def\wwc{\ww_{c}}

\def\norms{\circ} %{\vartriangle}
\def\rs{\rr_{\norms}}
\def\yys{\yy_{\norms}}
\def\xxs{\xx_{\norms}}
\def\zzs{\zz_{\norms}}
\def\uu{\mathtt{u}}
\def\uus{\uu_{\norms}}
\def\mus{\mu_{\norms}}
\def\gms{\gm_{\norms}}
\def\wws{\ww_{\circ}}

\def\srho{s}
\def\mrho{\varrho}
%\def\mrhoc{\mrho'}

\def\Lmgf{\mathfrak{M}}
\def\Lmgfb{\Lmgf^{*}}
%\def\LMGF{\cc{M}}
%\def\LMGFu{\LMGF_{*}}
%\def\Lmgfd{\bar{\Lmgf}}
%\def\LmgfP{\Lmgf^{\circ}}

\def\lmgf{\mathfrak{m}}
\def\lmgfb{\lmgf^{*}}
%\def\lmgfd{\bar{\lmgf}}


\def\Expzeta{\mathfrak{N}}
\def\expzeta{\mathfrak{s}}

%\def\Lexpm{\mathfrak{S}}
%\def\expzetab{\expzeta_{0}}
%\def\ExpL{\cc{D}}
%\def\mUU{\mathfrak{b}}
%\def\ExpL{d}
%\def\dI{\ExpL^{*}}
%\def\ExpM{\cc{M}}
%\def\fz{f}



%\def\rough{R}

\def\rr{\mathtt{r}}
\def\rrb{\rr^{*}}
\def\rru{\rr_{\circ}}
\def\rrc{\rr'}
\def\rs{r_{*}}

\def\zz{\mathfrak{z}}
\def\zzb{\tilde{\zz}}
\def\tt{\mathfrak{t}}
\def\zb{z_{\rd}}
\def\zzg{\zz_{1}}
\def\zzQ{\zz_{0}}
\def\zzq{\zz}

\def\Cr{\mathfrak{c}}
\def\Crp{\mathfrak{C}}
\def\Crl{\mathfrak{r}}
\def\Crlp{\mathfrak{R}}
%\def\Crlq{\mathfrak{T}}
\def\Crlq{\cc{T}}
%\def\Crlqc{\Crlq_{0}}
\def\Crlmu{\cc{M}}





%%%%%%%%%%%%   semipar   %%%%%%%%%%%%%%%%%%%%%%%%
\def\zetah{\zeta_{h}}
\def\GG{G}
\def\HH{H}
\def\pG{p}
\def\pH{q}
\def\hh{H^{*}}

\def\mubch{\mubc_{1}}
\def\rhoh{\rho_{1}}
\def\CoFuh{\CoFu_{1}}
\def\dimh{p_{1}}
\def\VPh{\VP_{1}}
\def\VPt{\VP_{0}}

\def\LLh{L_{1}}
\def\pnndh{\pnnd_{1}}

\def\LCS{C}
\def\Ac{A_{0}}
\def\Ab{A_{\rd}}
\def\DPrb{\DPr_{\rdb}}
\def\DPrm{\DPr_{\rdm}}
%\def\zetavrb{\zetavr_{\rd}}
\def\Cb{\cc{C}_{\rdb}}
\def\Ub{\cc{U}_{\rdb}}
\def\zetavrb{\zetavr_{\rd}}
\def\xivrb{\breve{\xiv}_{\rd}}
\def\VPrb{\breve{\VP}_{\rdb}}
\def\Larb{\breve{\La}_{\rdb}}
\def\Larm{\breve{\La}_{\rdm}}

\def\deltav{\bb{\delta}}

\def\score{\nabla}
\def\scorer{\breve{\nabla}}

\def\LCS{C}
\def\Ac{A_{0}}
\def\Bc{B_{0}}
\def\AF{A}
\def\Ab{A_{\rdb}}
\def\Am{A_{\rdm}}
\def\DPrc{\DPr_{0}}
\def\DPrb{\DPr_{\rdb}}
\def\DPrm{\DPr_{\rdm}}
\def\Cb{\cc{C}_{\rdb}}
\def\Cm{\cc{C}_{\rdm}}
\def\Ub{\cc{U}_{\rdb}}
\def\deltav{\bb{\delta}}
\def\nuv{\bb{\nu}}
%\def\scorer_{\thetav}{\zetavr_{\rd}}
\def\xivrb{\breve{\xiv}_{\rd}}
\def\VPrb{\breve{\VP}_{\rdb}}
\def\Larb{\breve{\La}_{\rdb}}
\def\Lar{\breve{\La}}
\def\Larm{\breve{\La}_{\rdm}}
\def\VH{Q}
\def\VHc{\VH_{0}}
\def\zetavrm{\zetavr_{\rdm}}
\def\N{\mathbb{N}}

\def\Span{\operatorname{span}}
\def\Exc{{\square}}
\def\UUs{U_{\circ}}
\def\errbm{\errb^{*}}
\def\corrDF{\nu}
\def\BBr{\breve{\BB}}
\def\taua{\tau}
\def\AssId{\mathcal{I}}
\def\assId{\iota}
\def\AFD{\cc{A}}

\def\BanX{\cc{X}}
\def\basX{\ev}
\def\apprX{\alpha}
\def\fvs{\fv^{*}}
\def\lkh{\ell}
\def\Bc{B_{0}}
\def\dimn{\dimp_{\nsize}}
\def\betan{\beta_{\nsize}}


%%%%%%%%%%%   BvM   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def\xivGP{\xiv_{\GP}}
\def\dimA{\mathtt{p}}
\def\dimAGP{\dimA}
\def\dime{\dimA_{e}}
\def\dimG{\dimA_{\GP}}
\def\dimS{\dimA_{s}}
\def\nubm{\nu_{\rd}}
\def\uub{u_{\rd}}
\def\uubGP{u_{\rd,\GP}}

\def\priorden{\pi}
\def\xivGP{\xiv_{\GP}}
\def\dimAGP{\dimA}
\def\nubm{\nu_{\rd}}
\def\uub{u_{\rd}}
\def\uubGP{u_{\rd,\GP}}

\def\CR{\mathcal{C}}
\def\CRb{\CR_{\rdb}}
\def\vthetavb{\bar{\vthetav}}
\def\Covpost{\mathfrak{S}}

\def\Db{\DP_{+}}
\def\Dm{\DP_{-}}
\def\uvb{\uv_{+}}
\def\uvm{\uv_{-}}
\def\uud{\omega}
\def\taub{\delta}
\def\Lip{L}
\def\Xb{X_{+}}
\def\Xm{X_{-}}
\def\deltam{\delta_{-}}
\def\betauv{\delta}
\def\betab{\betauv_{1}}
\def\betaf{\betauv_{2}}
\def\upsv{\bb{\varkappa}}
\def\upsvb{\bar{\upsv}}
\def\rhob{\varrho}
\def\alpb{\alp_{1}}
\def\betap{\betauv_{3}}
\def\Ec{\E^{\circ}}
\def\ff{f}
\def\fpos{g}
\def\fneg{h}
\def\alpb{\alp_{+}}
\def\alpm{\alp_{-}}




%%%%%%%%%%%   sms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\kappak{\kappa}
\def\kappas{\kappak^{*}}
\def\Kappak{\cc{K}}
\def\DPk{\DP_{\kappak}}
\def\VPk{\VP_{\kappak}}



%%%%%%%%%%%%   sp   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ts{s}
\def\tsv{\bb{\ts}}
%\def\mm{\kappa}
\def\mm{\varkappa}
\def\mms{\mm^{*}}
\def\mmc{\mm'}
\def\mmd{\mm^{\circ}}
\def\mmo{\mm^{*}}
\def\mmmmo{\mm,\mmo}
\def\mmt{\tilde{\mm}}
\def\mma{\hat{\mm}}
\def\mmcs{\mm_{c}}
\def\mmcmm{\mmc,\mm}
\def\mmcmmd{\mmc,\mmd}
\def\mmset{\mathcal{I}}
\def\mmz{\mm_{0}}
\def\bmm{\breve{\mm}}

\def\qqmd{\qq^{\circ}}


\def\pp{z}

\def\LLL{L_{1}}
\def\LLr{L_{0}}
\def\muL{\mu_{1}}
\def\mur{\mu_{0}}

\def\LmgfL{\Lmgf_{1}}
\def\Lmgfr{\Lmgf_{0}}
\def\Lmgfm{\Lmgf_{1}}

\def\Kappa{\cc{K}}
\def\CoFu{\cc{C}}
\def\CoFuc{\CoFu_{0}}
\def\CoFub{\CoFu^{*}}
\def\CoFuL{\CoFu_{1}}
\def\CoFur{\CoFu_{0}}
\def\CAL{\CA_{1}}
\def\CAr{\CA_{0}}
\def\CAzz{\cc{A}}

\def\pnnL{\pnn_{1}}
\def\pnnr{\pnn_{0}}
\def\ttd{\delta}
\def\alphaL{\alpha_{1}}
\def\alphar{\alpha_{0}}
\def\alpharL{\alpha}
\def\rat{\mathfrak{t}}
\def\mquad{\nquad}
\def\zzL{\zz_{1}}
\def\zzr{\zz_{0}}

\def\xex{u}
\def\dcm{q}
\def\dc{g}
\def\dcL{\dc_{1}}
\def\dcr{\dc_{0}}
\def\kk{k}

\def\cpen{\tau}

%=================  density  ==============
\def\dens{f}
\def\jj{j}
\def\JJ{\cc{J}}
\def\Zphi{Z}
\def\Zphiv{\bb{\Zphi}}


%================= LES =====================
\def\nuu{\mathfrak{u}}
\def\nud{\mathfrak{u}_{0}}
\def\nun{c_{\nuu}}
\def\rhork{\kullb}
\def\GH{\mbox{GH}}
\def\HYP{\mbox{HYP}}
\def\NIG{\mbox{NIG}}
\def\IR{{\rm I\!R}}
\def\taggr{b}
\def\penm{\boldsymbol{m}}
\def\Crlp{\cc{R}}

%================== qfu/cmr ====================
\def\Mh{M}
%\def\Mht{\tilde{\Mh}}
\def\Mht{\Mh^{c}}

\def\Mhh{\Mh^{-}}
\def\Mhc{G}
\def\Lh{L_{1}}
\def\Uh{\cc{U}}
\def\wloc{w}
\def\Bias{B}
%\def\bias{b}
\def\ExpzetaU{\Expzeta_{1}}
\def\vpci{\vp_{i,0}}
\def\IFci{\IF_{i,0}}

\def\erqb{\Circle_{\rdb}}
\def\erqm{\Circle_{\rdm}}
\def\errqm{\errm^{*}}
\def\errqb{\errb^{*}}
\def\Nsize{N}
\def\VVD{\VV_{1}}
\def\AA{A}
\def\Wloc{W}

%%%%%%%%%%%   rough   %%%%%%%%%%%%%
\def\tups{\pen_{0}}
\def\rupd{\rr_{\circ}}
\def\VVb{\VVc}
\def\BP{B}
\def\bp{b}

\def\gps{s}
\def\GK{\cc{G}}

\def\zzGP{\zz_{\GP}}

\def\entrlq{\entrl_{1}}
\def\entrlg{\entrl_{2}}
\def\kb{k^{*}}


\def\rderr{\chi}
\def\Excgr{\diamondsuit}
\def\Excgrb{\diamondsuit^{*}}
%\def\thetavs{\thetav_{0}}
\def\Thetat{\bar{\Theta}}
\def\biasGP{\bias_{\GP}}
\def\QL{W}
\def\QLG{\mathcal{W}}
\def\BPGP{\QLG_{\GP}}
\def\BBGP{\BB_{\GP}}

\def\xxn{\xx_{\nsize}}
\def\fisGP{\mathtt{w}_{\GP}}
\def\risktGP{\riskt_{\GP}}

\def\dimq{q}
\def\nul{\mathrm{o}}
\def\Thetan{\Theta_{\nul}}
\def\thetavn{\thetav_{\nul}}
\def\thetavsn{\thetavs_{\nul}}
\def\tilden#1{\tilde{#1}_{\nul}}
\def\tildeGP#1{\tilde{#1}_{\GP}}
\def\xivn{\xiv_{\nul}}
\def\xivrGP{\xivr_{\GP}}
\def\DPcc{\DP_{\nul}}
\def\DPnGP{\DP_{1,\GP}}
\def\DPnGPr{\breve{\DP}_{1,\GP}}
\def\nablan{\nabla_{\nul}}
\def\scoren{\score_{\nul}}
\def\AnGP{A_{\nul,\GP}}

\def\testst{T}
\def\TGP{\testst_{\GP}}

\def\VPD{\VP_{2}}

\def\entrlB{\entrl_{1}}
\def\SB{W}
\def\dimq{q}
\def\QQ{\mathbb{H}}
\def\QQg{\QQ_{2}}
\def\QQq{\QQ_{1}}
\def\FF{F}
\def\LaGP{\La_{\GP}}

\def\zzQ{\zz_{\QQ}}
\def\zzAA{\zz_{\FF}}
\def\zzAAA{\zz_{\FF,\SB}}
\def\cdimc{\cdima}
\def\fisGP{\fis_{\GP}}
\def\rdomegab{\rdomega^{*}}

\def\lambdaGP{\lambda_{\GP}}
\def\wGP{\mathrm{w}_{\GP}}


\def\uudm{\mathtt{w}}
\def\lambdaB{\lambda_{\BB}}

\def\lambdav{\bb{\lambda}}
\def\etavd{\etav_{\circ}}
\def\thetavb{\breve{\thetav}}
\def\vthetavd{\Ec \vthetav}
%\def\vthetavd{\bar{\vthetav}_{\circ}}
\def\Covd{S_{\circ}}
\def\Covpostd{\Covpost_{\circ}}
\def\IS{\mathcal{I}}
\def\etas{\eta^{*}}
\def\Po{\operatorname{Po}}
\def\IF{\Bbb{F}}
\def\etavb{\bar{\etav}}
\def\etavd{\etav^{\circ}}
\def\Pc{\P^{\circ}}
\def\xxn{\xx_{\nsize}}
\def\CRd{\CR^{\circ}}

\def\CONST{\mathtt{C} \hspace{0.1em}}

\def\dimB{\mathtt{p}_{\BB}}

\def\nub{\nu}
\def\VPD{\VP_{2}}
\def\SB{W}
\def\dimq{q}
\def\dimqb{\dimq^{*}}
\def\QQ{\mathbb{H}}
\def\QQg{\QQ_{2}}
\def\QQq{\QQ_{1}}
\def\FF{F}

\def\qq{z}
\def\qqBB{\qq_{\BB}}
\def\qqQ{\qq_{\QQ}}
\def\qqAA{\qq_{\FF}}
\def\qqAAA{\qq_{\FF,\SB}}
\def\rderr{\chi}
\def\Excgr{\diamondsuit}

\def\Ccb{m}
\def\Ccm{m}
\def\BB{B}

\def\vthetavd{\vthetav^{\circ}}
\def\Indru{\Ind_{\rups}}

\def\BBh{U}
\def\DD{U}
\def\hsp{\tau}
\def\fiD{a}

\def\Prior{\Pi}
\def\prior{\pi}

\def\In{\mathcal{I}}
\def\KK{\cc{K}}
\def\qqu{\qq^{*}}
\def\ws{\omega}




\def\Xs{X^{*}}
\def\Xvs{\Xv^{*}}
\def\Xvg{\Xv_{\gammav}}
\def\Upsilons{\Upsilon_{0}}


\def\DPE{\mathrm{D}}
\def\DLS{\Lambda_{\sigma}}
\def\DFtt{\DF_{\thetav\thetav}}
\def\DFXX{\DF_{\etav\etav}}
\def\AtX{A_{\thetav\etav}}
\def\VPD{\VF_{2}}
\def\VX{\VP_{2}}
\def\vx{\mathtt{v}}
\def\vp{\mathrm{v}}
\def\dpe{\mathrm{d}}

\def\AB{B}

\def\Tau{\mathscr{T}}
\def\Taus{\Tau_{\sigma}}
\def\eigIF{\mathtt{f}}
\def\CNiGP{N_{\GP}^{(1)}}
\def\CNiiGP{N_{\GP}^{(2)}}
\def\CNsGP{N_{\GP}^{(s)}}

\def\CQX{\CONST_{\phi}}

\def\rupsGP{\rr_{\GP}}
\def\ExcGP{\err_{\GP}}

\def\GPc{\GP'}
\def\LGPc{L_{\GPc}}

\def\GPs{\GP^{*}}
\def\DPGPs{\DP_{\GPs}}
\def\xivGPs{\xiv_{\GP}^{\circ}}
\def\biasGPs{\bias_{\GPs}}
\def\GPF{\cc{\GP}}

\def\biasGPGPc{\bb{\bias}_{\GP,\GPc}}
\def\DPGPc{\DP_{\GPc}}
\def\DPDPc{\DP_{\GP,\GPc}}
\def\MM{\cc{X}}

\def\qqm{\qq^{-}}
\def\qqmu{\qqm_{2}}
\def\qqu{\qq^{+}}

\def\biasu{\beta}

\def\biasQL{\bias^{{\QL}}}
\def\GPGPc{\GP,\GPc}
\def\GPd{\GP^{\circ}}

\def\qqQL{\qq^{{\QL}}}
\def\qqQLu{\qq^{+}}
\def\qqmm{\qqm_{\mm}}

\def\Omegas{\Omega^{+}}
\def\Excgru{\Excgr^{+}}
\def\ExcGPu{\ExcGP^{+}}


\def\kkd{\kk^{\circ}}
\def\kkc{\kk'}
\def\kks{\kk^{*}}

\def\lossu{\loss^{+}}
\def\risku{\riskt^{+}}

\def\codd{\, | \,}
%\def\als{\alpha}
\def\als{a}
\def\Als{s}

\def\ws{\Lambda}

\def\MMplus{\MM^{2}_{+}}

\newcommand{\omegasn}[1]{\omega_{\dimp,#1}}

%%%%%%%%%%%%%%%%   GAR   %%%%%%%%%%%%%%%
\def\teps{\tilde{\varepsilon}}
\def\epsb{\varepsilon^{\flat}}
\def\tepsv{\tilde{\epsv}}
\def\eps{\varepsilon}
\def\qqv{\bb{\qq}}
\def\tx{\tilde{x}}
\def\txv{\tilde{\xv}}
\def\txi{\tilde{\xi}}
\def\txiv{\tilde{\xiv}}
\def\tSv{\tilde{\Sv}}


%\def\betac{\beta_{1}}
\def\betac{b}
\def\Cfs{B}
\def\Meta{\mathbb{M}}
\def\Geta{\mathbb{G}}

\def\Wv{\bb{W}}
%\def\fm{s}
\def\fm{f}

\def\errXY{\, \Box}
\def\QXY{\mathbb{Q}}
\def\DeltaS{\Delta_{\Sigma}}

\def\ddv{U}
\def\deltan{\delta_{n}}

\def\up{u}
\def\Deltab{\bb{\Delta}}
%\def\fsp{\fs^{+}}
%\def\fsm{\fs^{-}}

\def\rrx{\rr_{x}}

\def\VPb{\cc{V}}
\def\QQb{\cc{H}}

\def\Cf{\mathtt{C}_{\fs}}
\def\sigml{\underline{\sigma}}
\def\sigmu{\bar{\sigma}}

\def\DS{\cc{G}}
\def\Deps{\Delta}
\def\qqY{\qq}
\def\qqz{z^{*}}
\def\Sigmab{\Sigma^{\sbt}}
\def\errxi{\Delta}
\def\errSi{\errXY}


\def\IFr{\breve{\IF}}
\def\Proa{\mathbb{H}_{1}}
\def\Pron{\mathbb{H}_{0}}
\def\bT{T^{\sbt}}
\def\bxivr{\breve{\xiv}^{\sbt}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%   bootstrap MS   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\sbt{\circ}

\def\Pb{\P^{\sbt}}
\def\Eb{\E^{\sbt}}
\def\bw{u}
%\def\bw{w^{\sbt}}
\def\bzeta{\zeta^{\sbt}}
\def\beps{\varepsilon^{\sbt}}
\def\berr{\err^{\sbt}}
\def\brhor{{\rhor^{\sbt}}}
\def\bxi{\xi^{\sbt}}
\def\bxiv{\xiv^{\sbt}}
\def\bSv{\Sv^{\sbt}}

%\def\mmmax{\bar{\mm}}
\def\mmmax{\mathtt{M}}
\def\md{\mm^{\circ}}
%\def\sbt{\, \sharp}
%\def\sbt{\#}
\def\sbt{\hspace{1pt} \flat}
%\def\sbt{\lozenge}%{\smallsquare}
\def\wb{u^{\sbt}}
\def\thetavbt{\tilde{\thetav}^{\sbt}}
\def\Tmdb{\Tmd^{\sbt}}
\def\xivb{\xiv^{\sbt}}
\def\zqb{\zq^{\sbt}}
\def\nB{B}
\def\Wb{\uv^{\sbt}}
\def\WB{\Uv^{\sbt}}
%\def\Ev{\bb{E}}
\def\epsvb{\epsv^{\sbt}}
\def\Varb{\Var^{\sbt}}
\def\Yvb{\Yv^{\sbt}}
\def\Yb{Y^{\sbt}}
\def\scoreb{\score^{\sbt}}
\def\VPb{{\VP^{\sbt}}}
\def\vB{\mathtt{v}}

%%%%%%%%%%%%%%%%%%%%%%%%%  single-index  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\xvd{\xv^{\circ}}
\def\yvd{\yv^{\circ}}
\def\gs{g}
%\def\IFone{F}
\def\IFone{\mathsf{H}}
\def\EPhi{\E_{\Phi}}
\def\Tv{\mathsf{T}}
\def\Av{\mathsf{A}}
\def\Tvs{\Tv_{0}}
\def\Phiv{\bb{\Phi}}
\def\PsiT{\mathsf{M}_{0}}
\def\PsiE{{\cc{M}}}
\def\psiM{\mathsf{m}}
\def\PsiV{{\mathsf{V}}}
\def\psiV{\mathsf{v}}
\def\usup{\mathsf{u}_{1}}
\def\Fr{\operatorname{Fr}}
%\def\CEDs{\mathsf{M}}
\def\ED{E\!D}
\def\Deltaf{\Delta_{\fv}}
\def\oper{\operatorname{op}}
\def\IFno{\IF_{0}}
\def\VPr{\breve{\VP}}
\def\VPno{\VP_{0}}
\def\vpno{\vp_{0}}
\def\fno{\mathsf{\vp}}
\def\Fno{\mathsf{H}}
\def\tups{\tau}
\def\tupsv{\bb{\tups}}
\def\VW{S}


\def\xxp{\xx_{\dimp}}
\def\xxnp{\xx_{n\dimp}}
\def\UV{\mathcal{U}}
\def\UVt{\mathcal{U}^{\T}}

\def\WP{W}
\def\MM{\cc{M}}
\def\MMu{\MM^{+}}
\def\MMd{\MM^{-}}
\def\MMi{\MM^{\circ}}
\def\NMMi{N^{\circ}}
\def\MMc{\MM^{c}}
\def\NMMc{N^{c}}
\def\msize{\mm}
%\def\mm{\mathbbmss{m}}
\def\mm{m}
\def\ms{\mm^{*}}
\def\mmb{\mm^{-}}
\def\mc{\mm'}
\def\mmmax{\mm_{\max}}
\def\jc{j'}
\def\md{\mm^{\circ}}
\def\xxm{\xx_{\msize}}
\def\xxb{\bar{\xx}}
\def\xxu{\xx^{c}}
\def\kku{\kk^{+}}
\def\kkm{\kk^{-}}
\def\kkb{\kk^{*}}
\def\qq{q}
\def\zzu{\zz^{+}}
\def\zzm{\zz^{-}}
\def\ZZu{\ZZ_{\alpb}}
\def\ZZm{\ZZ^{-}}
\def\ZZb{\bar{\ZZ}_{\alpb}}
\def\Deltau{\Delta^{+}}
\def\Deltam{\Delta^{-}}
\def\RMM{R}
\def\Tmmd{T}
\def\qqb{\qq^{*}}
%\def\ZZ{\mathtt{z}}
\def\ZZ{\mathtt{z}}
\def\ZZ{\mathfrak{z}}
\def\zq{z}
\def\zqb{\bar{\zq}}
\def\zND{z_{1}}
\def\zqu{\zq^{+}}
%\def\zpm{z^{\pm}}
\def\zpm{\zq^{\pm}}
\def\zqm{\zq^{-}}
\def\zqr{\mathtt{z}}
\def\RR{\cc{Q}}
\def\DQ{\cc{D}}
\def\VQ{\mathbb{V}}
\def\vq{\mathtt{s}}

\def\Tmd{\mathbb{T}}

%\def\dimq{\mathfrak{q}}
%\def\dimq{\mathtt{q}}
\def\dimq{q}
\def\alpb{\beta}
\def\alpd{\bar{\alp}}
\def\phis{\phi^{*}}
\def\biasm{b}
\def\riskr{\riskt^{+}}
\def\complx{\tau}
\def\ks{k^{*}}
\def\ZZb{\bar{\ZZ}}
\def\mmr{\breve{\mm}}

\def\thetavss{\thetav^{\star}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%   def   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\mmmax{\bar{\mm}}
%\def\mmmax{\mathtt{M}}
%\def\sbt{\, \sharp}
%\def\sbt{\#}
\def\sbt{\hspace{1pt} \flat}
%\def\sbt{\lozenge}%{\smallsquare}
\def\thetavbt{\tilde{\thetav}^{\sbt}}
\def\Tmdb{\Tmd^{\sbt}}
\def\xivb{\xiv^{\sbt}}
\def\zqb{\zq^{\sbt}}
\def\nB{B}
\def\wb{w^{\sbt}}
%\def\wbr{\epsilon^{\sbt}}
\def\wbr{e^{\sbt}}
\def\Wb{\wv^{\sbt}}
\def\WB{\cc{W}^{\sbt}}
\def\WBr{\cc{E}^{\sbt}}
%\def\Ev{\bb{E}}
\def\epsvb{\epsv^{\sbt}}
\def\Varb{\Var^{\sbt}}
\def\Yvb{\Yv^{\sbt}}
\def\Yb{Y^{\sbt}}
\def\scoreb{\score^{\sbt}}
\def\VPb{{\VP^{\sbt}}}
\def\vB{\mathtt{v}}
\def\dimAb{\dimA^{\sbt}}
\def\maxPsii{\dPsi}
\def\XX{\cc{X}}
\def\AEB{\bb{A}}
\def\Bias{\bb{B}}
\def\sigmab{\bar{\sigma}}
\def\dPsi{\delta_{\Psi}}
\def\tdPsi{\dPsi}
\def\aPsi{a_{\Psi}}
\def\aSigma{a_{\Sigma}}
\def\PPsi{\mathbb{Q}}
\def\PPsib{\mathbb{Q}^{\sbt}}
\def\DeltaPsi{\Delta}
\def\GW{G}
\def\VPB{\cc{V}}
\def\Xvb{\Xv^{\sbt}}

\def\AGLM{A}
\def\AGLMb{\AGLM^{\sbt}}

\def\vpb{{\vp^{\sbt}}}
\def\zetavb{\zetav^{\sbt}}
\def\scorebr{\breve{\score}^{\sbt}}
\def\epsvr{\breve{\epsv}}
\def\epsr{\breve{\eps}}
\def\kk{m}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%   end-def   %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pen{\mathtt{pen}}
\def\Sphere{\cc{S}}
\def\bvb{\bv^{\sbt}}
\def\bvs{\bv}
%\def\supA{\mathtt{a}}
\def\supA{\lambda}
\def\mmmin{\mm_{0}}
\def\mres{\breve{\mm}}
%\def\mmax{\mmmax}
\def\td{\delta}
\def\dimB{\dimA}
\def\vpB{\vp}
\def\lambdaB{\supA}
\def\zqc{\zq_{c}}


\def\totalpar{\phiv}
\def\totalpars{\totalpar^{*}}

\def\phivs{\phiv^{*}}
\def\nuisance{\phiv}
\def\nuisances{\phivs}
\def \nuisancesGP{\nuisances_{\GP}}
\def\upssGP{\upss_{\GP}}

\def\theteta{\upsilonv}
\def\thetavcut{\thetav,s}
\def\cutpar{\bb{\kappa}}
\def\cutpars{\cutpar^{*}}
\def\cutparkm{\cutpar}
\def\cutparskm{\cutpars}


\def\thetavss{\thetavs_{s}}
\def\thetavds{\thetavd_{s}}
\def\etavss{\etavs_{s}}
\def\etavskm{\etavs}
\def\upsm{\ups^{s}}
\def\thetetass{\thetetas_{s}}
%\def\thetavss{\thetav^{*s}}
%\def\thetavds{\thetav^{\circ s}}
%\def\etavss{\etav^{*s}}
%\def\thetetass{\theteta^{*s}}
\def\thetetas{\theteta^{*}}
\def\xivrs{\xivr_{s}}
\def\xivm{\xiv^{s}}

\def\thetavsm{\thetav^{s}}
\def\etavsm{\etav^{s}}
\def\etavkm{\etav}
\def\KM{\cc{S}}

%\def\xivrs{\xivr^{s}}
\def\biasc{\rho}
\def\biasp{b}
\def\ggdelta{\biasp_{\cutpar}}
\def\ggtheta{\biasc_{\cutpar}}
\def\km{m}
\def\ggdeltam{\biasp_{\km}}
\def\ggthetam{\biasc_{\km}}
\def\ggthetaGP{\biasc_{\GP}}
\def\ggdeltaGP{\biasp_{\GP}}
\def\VRF{\cc{E}}
\def\DPr{\breve{\DD}}
\def\DD{\mathbb{D}}
\def\DPs{\DP}
\def\DFs{\DF_{s}}
%\def\DPrs{\breve{\IFs}}
\def\DPrs{\mathbb{\DPs}}
\def\DFr{\breve{\DF}}


\def\CF{C}
\def\AP{A}
\def\AF{\cc{A}}


\def\alps{\alpha}
\def\rupc{\rr_{\cutpar}}
\def\rupm{\rr_{\km}}
%\def\scorers{\underline\scorer}
\def\AssIds{\AssId_{s}}
\def\scorers{\scorer}

%\def\IF{F}
\def\IFGP{\IF_{\GP}}
\def\DFGP{\DF_{\GP}}
\def\IFrm{\check{\IF}}

\def\IFt{\mathcal{F}}
\def\IFr{\IFt}
\def\IFs{\IFt_{\km}}
\def\IFsr{\IFt_{\km,\thetav}}


\def\xivrs{\breve{\xiv^{s}}}

%\def\AssIds{\AssId^{s}}
\def\EX{\E_{X}}



\def\tar{\phi}
\def\tars{\tar^{*}}
\def\tarv{\bb{\tar}}
\def\tarvs{\tarv^{*}}

\def\Tam{\cc{K}}

\def\test{\tau}

\def\ZZs{\bar{\ZZ}}
\def\ZZbt{\ZZ^{\sbt}}
\def\qqbt{\qq^{\sbt}}
\def\dimAbt{\dimA^{\sbt}}
\def\xxt{t}
\def\Yr{\breve{Y}}
\def\Yvr{\breve{\Yv}}
\def\mres{\mm^{\dag}}
\def\Sam{\cc{T}}
\def\epsb{\eps^{\sbt}}
\def\Varxi{S}
\def\Varxib{S^{\sbt}}
\def\dPi{\td_{\Pi}}
\def\dimPi{\dimA_{\Pi}}

\def\rei{\delta}
\def\vpi{\mathtt{b}}
\def\dPsis{\delta^{*}}
\def\BBB{\cc{B}}

\def\Covm{\Sigma}
\def\covm{\sigma}
\def\supAB{\supA^{*}}

\def\supepsi{\delta_{\eps}}
\def\supeps{\delta_{1}}
\def \UVcol{\bb{\omega}}
\def\Covm{\mathbb{V}}


==> bernulli2020(4)/subG.tex <==
\begin{lemma} \cite{HDStats} \label{sub_g_m}
Consider sub-Gaussian random variable $\xi$: 
\[
\log \E e^{\lambda \xi} \leq \frac{\nu^2 \lambda^2}{2}
\]
For $q \geq 2$
\[
[\E |\xi|^q]^{1/q} \leq    \nu e^{1/e} q^{1/2}
\]
and 
\[
\E |\xi| \leq \nu \sqrt{2\pi}
\]
\end{lemma}

==> bernulli2020(4)/task_def.tex <==
Having introduced the main definitions in the previous section, we want to find an upper bound for $ | \normx{\xiv}  - \normx{\gammav} |$  in probability. 
Markov's inequality gives the following for some $L \geq 0$:
\[\label{ME}
\P \left ( \left| \normx{\xiv}  - \normx{ \gammav } \right|  > \Delta \right) 
\leq \P \left( \normx{\xiv - \gammav }  > \Delta \right) 
\leq \frac{\E \normx{\xiv - \gammav }^L}{\Delta^L}. 
\]
The differences $ \normx{ \xiv  -  \gammav }$ decrease when the dependence between the random variables increases. So we want to make them as dependent as possible.
Denote by $\pi(\xiv, \gammav)$ a joint distribution of $\xiv$ and $\gammav$. 
One then has to minimize over $\pi$ with a fixed marginals ($\pi \in \Pi[\xiv, \gammav]$) the following Wasserstein distance 
\begin{equation}\label{equation_3}
W_L^L(\xiv, \gammav) = \min_{\pi \in \Pi[\xiv, \gammav]} \left\{ \E  \| \xiv  - \gammav \|^L \right\}.
\end{equation}
\noindent Notation $\pi \in \Pi[\xiv, \gammav]$ means that $\int \pi(\xiv, d \gammav) $ equals the distribution of $\xiv$ and $\int \pi(d \xiv, \gammav) $ equals the distribution of $\gammav$. Accounting to the previous inequalities,
\begin{equation} \label{markov_bound}
\min_{\pi \in \Pi[\xiv, \gammav]} \P \left(  \left| \normx{\xiv}  - \normx{ \gammav } \right|> \Delta \right) \leq  \frac{W_L^L(\xiv, \gammav)} {\Delta^L}. 
\end{equation}
Below, we will study one/multi dimensional cases separately because of the difference in the complexity of the proof.    An accurate solution of this problem is applicable for a lot of different fields of science \cite{NIPS2013_cuturi, Chernozhukov, cpd_boot, cpd_ecg} and thus so important.


==> subG.tex <==
\begin{lemma} \cite{HDStats} \label{sub_g_m}
Consider sub-Gaussian random variable $\xi$: 
\[
\log \E e^{\lambda \xi} \leq \frac{\nu^2 \lambda^2}{2}
\]
For $q \geq 2$
\[
[\E |\xi|^q]^{1/q} \leq    \nu e^{1/e} q^{1/2}
\]
and 
\[
\E |\xi| \leq \nu \sqrt{2\pi}
\]
\end{lemma}
